Practical Data Compression for Modern Memory Hierarchies

In this thesis, we describe a new, practical approach to integrating hardware-based data compression within the memory hierarchy, including on-chip caches, main memory, and both on-chip and off-chip interconnects. This new approach is fast, simple, and effective in saving storage space. A key insight in our approach is that access time (including decompression latency) is critical in modern memory hierarchies. By combining inexpensive hardware support with modest OS support, our holistic approach to compression achieves substantial improvements in performance and energy efficiency across the memory hierarchy. Using this new approach, we make several major contributions in this thesis. First, we propose a new compression algorithm, Base-Delta-Immediate Compression (BDI), that achieves high compression ratio with very low compression/decompression latency. BDI exploits the existing low dynamic range of values present in many cache lines to compress them to smaller sizes using Base+Delta encoding. Second, we observe that the compressed size of a cache block can be indicative of its reuse. We use this observation to develop a new cache insertion policy for compressed caches, the Size-based Insertion Policy (SIP), which uses the size of a compressed block as one of the metrics to predict its potential future reuse. Third, we propose a new main memory compression framework, Linearly Compressed Pages (LCP), that significantly reduces the complexity and power cost of supporting main memory compression. We demonstrate that any compression algorithm can be adapted to fit the requirements of LCP, and that LCP can be efficiently integrated with the existing cache compression designs, avoiding extra compression/decompression.

==> Makefile <==
# Set this to "off" to use normal LaTeX:
USE_PDFLATEX = true

MAINFILE = main.tex

SUBFILES = $(wildcard chap*.tex) $(wildcard chap*/*.tex) 

# xfig drawings to be included in the document
FIGFILES = $(wildcard fig/*.fig) $(wildcard chap*/graphs/*.fig)

# other postscript files to be included in the document
EPSFILES = $(wildcard eps/*.eps) $(wildcard chap*/graphs/*.eps)

BIBFILES = $(wildcard *.bib)

# constants

MAKE = make --no-print-directory 

MAIN = $(subst .tex,,$(MAINFILE))
MAINBBL = $(MAIN).bbl
MAINPS = $(MAIN).ps
MAINPDF = $(MAIN).pdf
ifeq ($(USE_PDFLATEX),true)
MAINDVI = $(MAIN).pdf
OUTPUT = $(MAINPDF)
else
MAINDVI = $(MAIN).dvi
OUTPUT = $(MAINPS)
endif
MAINAUX = $(MAIN).aux
MAINTOC = $(MAIN).toc
MAINLOG = $(MAIN).log

ifeq ($(USE_PDFLATEX),true)
latex = pdflatex
else
latex = latex
endif

bibtex = bibtex
fig2dev = fig2dev
printer = stone
gv = kghostview

# file where we measure our progress by bytes, words, lines and pages
WCLOGFILE = $(MAIN).wc
REBIBFLAG = $(MAIN).must_remake_bbl.flag


# COMMANDS

.PHONY: dvi ps print xdvi gv backup clean grep latex_doit bibtex_doit

all:	$(OUTPUT)

dvi:	$(WCLOGFILE)

ps:	dvi $(MAINPS)

pdf:	$(MAINPDF)

print:	ps
	lpr -P$(printer) $(MAINPS)
	lpq -P$(printer)

xdvi:	dvi
	xdvi -s 4 $(MAINDVI)

gv:	$(OUTPUT)
	$(gv) $<

acroread: pdf
	acroread $(MAINPDF)

c1:
	$(MAKE) MAINFILE=chap1_alone.tex gv

c1_pdf:
	$(MAKE) MAINFILE=chap1_alone.tex acroread

c2:
	$(MAKE) MAINFILE=chap2_alone.tex gv

c2_pdf:
	$(MAKE) MAINFILE=chap2_alone.tex acroread

c3:
	$(MAKE) MAINFILE=chap3_alone.tex gv

c3_pdf:
	$(MAKE) MAINFILE=chap3_alone.tex acroread

c4:
	$(MAKE) MAINFILE=chap4_alone.tex gv

c4_pdf:
	$(MAKE) MAINFILE=chap4_alone.tex acroread

c5:
	$(MAKE) MAINFILE=chap5_alone.tex gv

c5_pdf:
	$(MAKE) MAINFILE=chap5_alone.tex acroread

app:
	$(MAKE) MAINFILE=appendix_alone.tex gv

app_pdf:
	$(MAKE) MAINFILE=appendix_alone.tex acroread

backup:
	test -d backup || mkdir backup
	tar cvf backup/`date +%y-%m-%d`.tar Makefile NOTES $(MAINFILE) $(SUBFILES) $(FIGFILES) $(EPSFILES) $(BIBFILES) $(WCLOGFILE) ; gzip -f backup/*.tar

clean:	
	rm -f *.dvi
	rm -f *.aux
	rm -f *.log
	rm -f *.toc
	rm -f *.lof
	rm -f *.lot
	rm -f *.idx
	rm -f *.ind
	rm -f *.ilg
	rm -f *.bbl
	rm -f *.blg
	rm -f *.toc.copy
	rm -f $(FIGFILES:.fig=.eps)
	rm -f $(FIGFILES:.fig=.pdf)
	rm -f $(EPSFILES:.eps=.pdf)
	rm -f $(MAINPS)
	rm -f *~
	rm -f main.pdf 
	rm -f main.out 
	rm -f main.brf 




# e.g. gmake grep string='traveling salesman'
grep:
	@echo '*****' Searching for '"'$(string)'"' in thesis files '*****'
	@fgrep -i -e '$(string)' $(MAINFILE) $(SUBFILES) $(BIBFILES)


# RULES

# kill some default rules
.SUFFIXES:

$(WCLOGFILE):	$(MAINDVI)
	./bin/wordcount $(MAIN) >> $(WCLOGFILE)
        # after every successful compile, log word count to WCLOGFILE.

$(MAINDVI):	$(MAINFILE) $(SUBFILES) $(EPSFILES:.eps=.pdf) $(FIGFILES:.fig=.eps) $(FIGFILES:.fig=.pdf) $(MAINBBL)
	@echo === Running LaTeX for the first time ===
	$(MAKE) latex_doit
	@echo === Checking if we need to rebuild bibliography ===
	@./bin/nowarning 'citation.*undefined' $(MAINLOG) || touch $(REBIBFLAG)
	@(test -f $(REBIBFLAG) && ( echo === Building bibliography === ; $(MAKE) -k bibtex_doit latex_doit)) || true
#       Rerun if the post-latex ToC is not identical to the pre-latex one.
	@diff $(MAINTOC) $(MAINTOC).copy > /dev/null || (echo === Re-running LaTeX to update table of contents === ; $(MAKE) latex_doit)
	@./bin/nowarning 'rerun' $(MAINLOG) || (echo === Re-running LaTeX === ; $(MAKE) latex_doit)
	@./bin/nowarning 'rerun' $(MAINLOG) || (echo === Re-running LaTeX === ; $(MAKE) latex_doit)
	@./bin/nowarning 'warning' $(MAINLOG) || (echo === Re-running LaTeX due to warnings === ; $(MAKE) latex_doit)
	@echo  === Checking for errors ===
	./bin/tex_error $(MAINLOG)
#	@echo === Checking for warnings ===
#	./bin/nowarning 'warning' $(MAINLOG)

$(MAINBBL): $(BIBFILES)
	@echo === BibTeX files updated, must rebuild bibliography ===
	@touch $(MAINBBL)
	@touch $(REBIBFLAG)

latex_doit:
	@touch $(MAINTOC) ; cp -p $(MAINTOC) $(MAINTOC).copy
	-$(latex) '\nonstopmode\input{$(MAINFILE)}' >/dev/null
	./bin/tex_error -nw $(MAINLOG)

bibtex_doit:
	$(bibtex) $(MAIN)
	@rm -f $(REBIBFLAG)

%.eps : %.fig
	$(fig2dev) -L eps $< $@

%.pdf : %.eps
	epstopdf $< --outfile=$@

%.ps : %.dvi
	@echo === Converting DVI file to PostScript ===
	dvips -Ppdf -o $@ $< 2>/dev/null

%.pdf : %.ps
	@echo === Converting PostScript file to PDF ===
	ps2pdf -dAutoRotatePages=/None $<


==> README <==
This is a thesis template for CMU in latex2e format.
It is set up so that it can by hooked up to the thesisometer
system. Check out http://www.cs.cmu.edu/~jab/tom/ for details...

I don't guarantee that this is valid, hey, I haven't submitted
the thesis yet. So send comments to moi, josullvn@cs.cmu.edu

To build your thesis into a ps file, type "make ps".  To build it and
view it, type "make gv".  To build just a specific chapter, type "make
c1", "make c2", etc.

To change between making a PDF or a PS version of the thesis, type 
"make USE_PDFLATEX=true" or "make USE_PDFLATEX=false" (or just edit
the Makefile.)

Note that the cool date hack in the top left corner doesn't work for
PDF.  Darn.  :-(


March 7, 2005 (pfr)
        -> Use \frontmatter, \mainmatter, \appendix, \backmatter
        correctly (prevents page nubmering hacks)
        -> Use natbib for citations (including illustration of \citep
        and \citet)
        -> Use hyperref to get pdf bookmarks
        -> bin/tex_error: don't error out on pdfTeX warnings that look
        like errors
        -> Replaced ps specific draftstamp with draftstamp.sty

January 17 2005
        -> Added PDF support, various other improvements

November 18th 2003
        -> Stolen and updated by colohan

Feb 14th 2000
	-> Updated the rubber stamp thanks to ps wizard kosak
	-> changed the formatting thingy with some stuff from bnoble

Jan 29 2000
	-> a better heading style stolen from jrs via pdinda
	-> some rh6.1 stuff via me
	-> a neato draft rubber stamp, better than psdraft via caruana
	-> added \parskip=5pt (not certain about this)

Sept 9th 1999
	Original Version -- adapted from jab, mjz, millions.

Notes:
	bnoble   = Brian Noble
	caruana  = Rich Caruana
        colohan  = Chris Colohan
	jab      = Justin Boyan
	josullvn = Joseph O'Sullivan
	jrs      = Jonathan Shewchuk
	kosak    = Corey Kosak
	mjz      = Matt Zekauskas (mattz@cs)
	pdinda   = Peter Dinda
	pfr      = Patrick Riley


==> bin/nowarning <==
#!/usr/bin/perl
# -*-Mode: Perl;-*-

$regexp = shift;
$file = shift;

if (! -f $file) {
    die "Couldn't read log file [$file]\n";
}

$match = "m\"$regexp\"i";

$found_warn = 0;

open(F, $file);
while(<F>) {
    if (eval $match) {
	chop;
#	warn "
#-----------------
#Found warning [$regexp]:
#'$_'
#-----------------\n";
	$found_warn = 1;
    }
}
close(F);
exit($found_warn);


==> bin/tex_error <==
#!/usr/bin/perl
# -*-Mode: Perl;-*-

$file = shift;

if($file eq "-nw") {
    $nowarn = 1;
    $file = shift;
} else {
    $nowarn = 0;
}

if (! -f $file) {
    die "Couldn't read log file [$file]\n";
}

$curfile = "";
$curline = "";
$err = 0;
$found_err = 0;
$found_warn = 0;
$pfile = "";

open(F, $file);
while(<F>) {
    chomp;
    if(/^.*\(.*\.tex/) {
	$curfile = $_;
	$curfile =~ s/\.tex.*/.tex/;
	$curfile =~ s/^.*\(//;
	$curline = "";
    }
    if(/^l\.\d+/) {
	$curline = $_;
	$curline =~ s/^l\.(\d+).*/$1/;
    }
    if(/^\!/ && not /^\! pdfTeX warning/) {
	unless($pfile eq $curfile) {
	    print "-----------------\nFile $curfile\n";
	    $pfile = $curfile;
	}
	if($curline eq "") {
	    print "    $_\n";
	} else {
	    print "    $curline: $_\n";
	}

	$err = 1;
	$found_err = 1;
    } elsif($nowarn == 0 &&
	    (/^LaTeX Warning/ ||
            /^\! pdfTeX warning/)) {
	unless($pfile eq $curfile) {
	    print "-----------------\nFile $curfile\n";
	    $pfile = $curfile;
	}
	if($curline eq "") {
	    print "    $_\n";
	} else {
	    print "    $curline: $_\n";
	}
	$found_warn = 1;
    } elsif($err) {
	$err = 0;
	print "    $_\n";
    }
}
close(F);

if($found_warn || $found_err) {
    print "-----------------\n";
}

exit($found_err);


==> bin/wordcount <==
#!/usr/bin/perl

$tex = "$ARGV[0].tex";
$log = "$ARGV[0].log";

#chop($wc = `TEXINPUTS=. ; detex $tex | wc`);
#chop($wc = `TEXINPUTS=. ; cat $tex | wc`);

if (!open(LOG, $log)) {
    $pages = -1;
}
else {
    # read pagecounts from log file.
    $/ = "setting this thuswise means we'll slurp whole file into one line";
    while(<LOG>) {
	while (/\[\s*(\d+)\s*\]/g) {
	    $pages = $1;
	}
    }
}

$d = `date`;
chop($d);
print "$d  Pages= $pages\n";




###	echo `perl -e 'print time'` `TEXINPUTS=. ; detex ${MAINFILE} | wc` >> ${WCLOGFILE}


==> camp/font.tex <==
\usepackage[T1]{fontenc}
\usepackage{libertine}
\renewcommand*\oldstylenums[1]{{\fontfamily{fxlj}\selectfont #1}}


==> camp/sections/0_abstract.tex <==
\begin{abstract}
We introduce a set of new \emph{Compression-Aware Management Policies (\carp)}
 for on-chip caches that employ data compression. 
Our management policies are based on two key ideas. First, we show that it is 
possible to build a more efficient management policy for compressed caches
if the compressed block size is directly used in calculating the \emph{value (importance)} of a block
to the cache. This leads to \emph{Minimal-Value Eviction (MVE)}, a policy that evicts
the cache blocks with the least value, based on both the size and the expected future reuse.
Second, we show that, in some cases, compressed block size can be used as an efficient indicator 
of the future reuse of a cache block. We use this idea to build a new insertion policy 
called \emph{Size-based Insertion Policy (SIP)} that dynamically 
prioritizes cache blocks
using their compressed size as an indicator. 
%We incorporate both the \mineviction{} and \insertionpolicy{} policies to form the \emph{Compression-Aware Management Policy (\carp)}.

We compare \carp{} (and its global variant G-\carp{}) to prior on-chip cache management policies (both 
size-oblivious and size-aware) and find that our mechanisms are more effective 
in using compressed block size as an extra dimension in cache management decisions.  
Our results show that the proposed management policies 
(i) decrease off-chip bandwidth consumption (by 8.7\% in single-core), (ii) decrease
memory subsystem energy consumption (by 7.2\% in single-core) for memory
intensive workloads compared to the best prior mechanism, and (iii) improve performance
(by 4.9\%/9.0\%/10.2\% on average in single-/two-/four-core workload evaluations and up to 20.1\%)
%and by as much as 13.9\% / 11.3\% over the traditional compressed cache design with Least-Recently-Used
%(LRU) policy. 
%Our replacement policies signficantly decrease off-chip bandwidth consumption (by 12.2\%)
%and memory subsystem energy (by 7.8\%) on average across all applications when compared with
%the best prior mechanism.  
\carp{} is effective for a variety of compression algorithms and different cache designs  with local and global replacement
strategies.

\end{abstract}


==> camp/sections/10_ack.tex <==
\section*{Acknowledgements}

We thank the reviewers for their valuable suggestions. We thank Hadi Esmaeilzadeh from
Georgia Tech for
his helpful comments on earlier version of this paper. 
We thank the SAFARI group members for the feedback and
stimulating research environment they provide.
We acknowledge the support of our industrial partners: Facebook, Google, IBM, Intel, Microsoft, Qualcomm, VMware, and Samsung.
This research was partially supported by NSF (grants 0953246, 1212962, 1065112, 1423172), the Semiconductor Research Corporation and the Intel Science and Technology Center for Cloud Computing.
Gennady Pekhimenko is supported 
by a Microsoft Research Fellowship and a Qualcomm Innovation Fellowship.


==> camp/sections/2_motivation.tex <==
\section{Motivating Observations}
\label{sec:motivation}

%\begin{figure*}[!h]
%  \vspace{-0.4cm}
%  \centering
%  \includegraphics[width=0.90\textwidth]{figures/belady_example.pdf}
%  \caption{The downside of not including block size information in replacement decisions.}
%  \vspace{-0.2cm}
%  \label{fig:belady}
%\end{figure*}

Cache compression~\cite{fvc,fpc,bdi,iic-comp,c-pack} is a powerful mechanism that increases 
effective cache capacity and decreases off-chip bandwidth consumption. 
In this section, we show that cache compression adds an additional dimension
to cache management policy decisions -- \emph{the compressed block size} (or
simply \emph{the size}), which plays an important role in building more efficient management 
policies. We do this in three steps.

%Even with increased cache capacity, 
%efficient management of cached data is essential for maximizing performance. 
%In this section, it is first shown that 
%replacement decisions in compressed caches are improved by considering compressed cache block size along with temporal 
%locality to identify blocks to be evicted. Second, looking at cache compression reveals the challenges and opportunities involved in managing compressed caches.
%\REM{While
%these straightforward benefits of cache compression were studied in several
%recent works~\cite{bdi,c-pack,fpc}, very few works~\cite{ecm} look at the additional
%opportunities such as size-aware cache management policies created by cache compression.
%In this work, we show that cache compression adds an additional dimension
%to cache management policy decisions -- \emph{the compressed block size} (or
%simply \emph{the size}),
%that plays an important role in building more efficient management 
%policies. We do this in three steps. 
%}
%\textbf{Size matters.}
\subsection{Size Matters}
%\subsection{Impact of Cache Block Size on Replacement.}
%todo: add the footnote about MLP- unawareness
In compressed caches, replacement algorithms that take into account compressed cache block size along with locality to identify victim blocks can outperform existing policies that rely only on locality. 
In fact, Belady's optimal algorithm~\cite{belady} that relies only on locality (using perfect knowledge to evict the block that will be accessed furthest in the future) is sub-optimal in the context of compressed caches
with variable size cache blocks. 
Figure~\ref{fig:belady} demonstrates one possible example of such a scenario. In this figure, it is assumed that cache blocks are one of two sizes: 
\begin{inparaenum}[(i)]
\item uncompressed 64-byte blocks (blocks X and Y) and
\item compressed 32-byte blocks (blocks A, B, and C).
\end{inparaenum}
Initially (see \ding{202}), the 160-byte capacity cache contains four blocks: three compressed blocks (A, B, C) 
and one uncompressed block (Y). Consider the sequence of memory requests X, A, Y, B, and C (see  \ding{203}). In this case, after a request for X, Belady's algorithm (based on locality) will evict blocks B and C (to create 64-bytes of free space) that will be accessed furthest into the future. Over the next four accesses, this results in two misses (B and C) and two hits (A and Y). 

In contrast, a size-aware replacement policy can detect that it might be better to retain a set of smaller compressed cache blocks 
that receive more hits cumulatively than a single large (potentially uncompressed) cache block with better locality.
%The intuition is that multiple smaller blocks cumulatively can provide more hits than a single large cache block.
For the access pattern discussed above, a size-aware replacement policy makes the decision to retain B and C and evict Y to make space for X (see  \ding{204}). As a result, the cache experiences three hits (A, B, and C) and only one miss (Y) and hence outperforms Belady's optimal algorithm.\footnote{Note that if later (see  \ding{205}) there are three additional requests to blocks B, Y, and A (all three hits), the final
cache state becomes the same as the initial one. Hence, this example can represent steady 
state within a loop.} We conclude that using block size information in a compressed cache can lead to better replacement decisions. 
%~\footnote{In this paper, we assume that data is uncompressed in main memory.  Consequently, reducing miss rate results in a proportional reduction in memory bandwidth.  If, alternatively, compressed cache lines were stored in memory, 64 bytes of compressed data would be fetched under both policies in this example.  However, compression-aware replacement policies could yield {\em both} fewer misses and fewer bytes fetched than compression-oblivious policies in other situations.} 
%Note that if later (see  \ding{205}) there are three additional requests to blocks B, Y, and A (all three hits), the final
%cache state becomes the same as the initial one. Hence, this example can represent steady 
%state within a loop.  

\subsection{Size Varies}
Figure~\ref{fig:bdi} shows the distribution of compressed cache block 
sizes\footnote{Section~\ref{sec:methodology} describes the details of our evaluation 
methodology for this and other experiments.} for a set of representative workloads given a 2MB cache employing the BDI~\cite{bdi} cache compression algorithm 
(our results with FPC~\cite{fpc} compression algorithm show similar trends).  Even though the size of a compressed block is determined by the compression algorithm, 
under both designs, \textbf{compressed cache block sizes can vary significantly}, both 
\begin{inparaenum}[(i)]
\item within a single application (i.e., \emph{intra-application}) such as in \emph{astar, povray}, and \emph{gcc} and
\item between applications (i.e., \emph{inter-application}) such as between \emph{h264ref} and \emph{wrf}.
\end{inparaenum}

\begin{figure}[t]
  %\centering
  \centering
  \includegraphics[width=0.45\textwidth]{figures/distribution_bdi.pdf}
\caption{Compressed block size distribution for representative applications with the BDI compression algorithm.}
\vspace{-0.2cm}
\label{fig:bdi}
\end{figure}

\REM{
In order to show that compressed block sizes significantly vary both within 
and between
multiple applications, we conducted an experiment\footnote{Section~\ref{sec:methodology}
describes the details of our evaluation methodology for this and other experiments.} 
where we observed the cache block size distribution (collected from snapshots of the 2MB last-level-cache).
Figures~\ref{fig:bdi} and \ref{fig:fpc1} show the distributions of compressed block
sizes for a representative selection of applications from our workload pool.
In order to simplify both the data representation and analysis, we split
all possible sizes into 8-byte bins with one special bin for 64-byte (uncompressed)
blocks. 
We can draw two major conclusions from these figures.

First, the compressed block sizes vary significantly both 
(i) within an application (e.g., \emph{astar}), and
(ii) between the applications
(e.g., compare \emph{h264ref} and \emph{wrf}).
} 

Size variation within an application suggests that size-aware replacement policies could be effective for individual single-core workloads. 
Intra-application variation exists because applications have data that belongs
to different common compressible patterns (e.g., zeros, repeated values, and narrow values~\cite{bdi,fpc})
and as a result end up with a mix of compressed cache block sizes.
In the case of multiple cores with shared caches, inter-application variation suggests that even 
if an application has a single dominant compressed cache block size (e.g., \emph{lbm, h264ref} and \emph{wrf}), 
running these applications together will result in the shared cache experiencing a mix of compressed cache block sizes. 
Hence, size-aware management of compressed caches can be even more important for efficient cache utilization in multi-core systems (as
we demonstrate quantitatively in Section~\ref{sec:multicore}).

\REM{
Inter-application variation suggests that
even if there is no significant variation within some individual applications, size
can vary significantly when these applications share the compressed cache (which creates
opportunities for size-aware replacement).
For example, if two (or more) applications have a dominant compressed block size
(e.g., \emph{h264ref} and \emph{wrf}), there is usually 
significant size variation (as with the variation within an application) 
when these applications are running together in a system
with a shared compressed cache.


Second, although the compressed block size is inherently dependent on
the compression algorithm that is used in cache compression,
comparison of the distributions from figure~\ref{fig:bdi} and figure~\ref{fig:fpc1} 
allows us to claim that size variation exists for different
compression algorithms: BDI~\cite{bdi} and FPC~\cite{fpc}. In general, we 
expect that our observations about the size variation hold for other 
compression algorithms as well, e.g., C-pack~\cite{c-pack}, and hence
we expect that the mechanisms we build based on these observations (see Section~\ref{sec:mve}) 
will be general
enough to work with different cache designs and compression algorithms.
}


\subsection{Size Indicates Reuse}
\label{sec:size-reuse}
%The benefits of knowing the size are not limited
%to providing an extra dimension that can be used in our replacement
%policies (Section~\ref{sec:mve}) either. 

\textbf{Intuition.} 
%We observe that elements belonging to the same data structure (within an application) sometimes compress to the same size.
%This observation provides a new opportunity: using compressed size as an indicator of data reuse.
We observe that elements belonging to the same data structure (within
an application) sometimes lead to cache blocks that compress to the
same size.  This observation provides a new opportunity: using the
compressed size of a cache block as an indicator of data reuse. 
Typically an application's key data structures are accessed in a regular fashion, 
with each data structure having an identifiable access pattern~\cite{dataStructurePhase}. This regularity in accesses 
can lead to a dominant {\em reuse distance}~\cite{reuse} range for the cache blocks belonging to the data structure
(captured in some prior works~\cite{madcache,cachebasedonreusedist,singleUsage,DataCacheManagement} by 
learning the relationship between the instruction address and the reuse distance).
%be reflected in terms of predictable reuse distances of the cache blocks belonging to the data structures. 
%Some prior works capture this by learning the relationship between the PC (instruction address) 
%that accesses the data structure and the reuse distance~\cite{madcache,cachebasedonreusedist,singleUsage,DataCacheManagement}. 
%The key shortcoming of such solutions is the addition of new hardware to learn the correlation (if any) 
%between PC and reuse distance. 
The same data structure can also have a dominant compressed cache
block size, i.e., a majority of the cache blocks containing the data
structure can be compressed to one or few particular sizes. For such
a data structure, the compressed cache block size can therefore be a
good indicator of the reuse behavior of the cache blocks. In fact,
different data structures can have different dominant compressed block
sizes and different dominant reuse distances, enabling compressed
block size to be used as a ``signature'' that can indicate reuse
patterns of a data structure's cache blocks.

%On the other hand, if some key data structures have a dominant compressed size (i.e. a majority of the elements are compressed to one or few particular sizes), 
%this size can be used as a signature for these data structures.
%In such cases, regular access patterns to such data structures can be linked to (and hence be indicated by)
%the compressed size of the cache blocks that store these data structures.
%. and hence predictable reuse 
%distances correlate with the compressed cache block size.
%Another key observation that we make is that a specific compressed block size
%within an application frequently correlates with a particular data structure,
%e.g., a certain array of elements stored in the compressed cache
%will likely have the same compressed block size
%for its data elements. This observation creates 
%an interesting opportunity. If an application's key data structures have
%certain dominant compressed sizes and these data structures
%also have some special properties when stored in the compressed cache, e.g.,
%certain average reuse distance,
%then compressed block size can be used as a predictor of these properties. 
\textbf{Quantitative Evidence.}
To verify the relationship between the compressed size and reuse, 
we conducted an experiment with our applications' memory traces (23 memory intensive applications)
to look for the presence of a linkage between the compressed size and reuse.
For every block within an application, we computed the distance (measured in memory requests) 
between the time this block was inserted into the compressed
cache and the time when it was reused next. We then accumulate this information
for all different sizes.
%We then average the reuse distance across the compressed
%blocks of the same size. 

\begin{figure*}[t]
  \vspace{-0.7cm}
  \centering
  \begin{subfigure}[b]{0.33\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/bzip2.pdf}
  \vspace{-0.6cm}
  \caption*{\scriptsize{Size (bytes)}}
  \vspace{-0.2cm}
  \caption{bzip2}
  \label{fig:bzip2}
  \end{subfigure}
  %\hspace{0.1cm}
  \begin{subfigure}[b]{0.33\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/leslie3d.pdf}
  \vspace{-0.6cm}
  \caption*{\scriptsize{Size (bytes)}}
  \vspace{-0.2cm}
  \caption{leslie3d}
  %\vspace{-0.2cm}
  \label{fig:leslie3d}
  \end{subfigure}
  \begin{subfigure}[b]{0.33\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/gcc.pdf}
  \vspace{-0.6cm}
  \caption*{\scriptsize{Size (bytes)}}
  \vspace{-0.2cm}
  \caption{gcc}
  %\vspace{-0.2cm}
  \label{fig:gcc}
  \end{subfigure}
  %\vspace{-0.1cm}
  \begin{subfigure}[b]{0.33\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/sphinx3.pdf}
  \vspace{-0.6cm}
  \caption*{\scriptsize{Size (bytes)}}
  \vspace{-0.2cm}
  \caption{sphinx3}
  %\vspace{-0.2cm}
  \label{fig:sphinx3}
  \end{subfigure}
  %\hspace{0.1cm}
  \begin{subfigure}[b]{0.33\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/tpch6.pdf}
  \vspace{-0.6cm}
  \caption*{\scriptsize{Size (bytes)}}
  \vspace{-0.2cm}
  \caption{tpch6}
  %\vspace{-0.2cm}
  \label{fig:tpch6}
  \end{subfigure}
  \begin{subfigure}[b]{0.33\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/soplex.pdf}
  \vspace{-0.6cm}
  \caption*{\scriptsize{Size (bytes)}}
  \vspace{-0.2cm}
  \caption{soplex}
  %\vspace{-0.2cm}
  \label{fig:soplex}
  \end{subfigure}
  \begin{subfigure}[b]{0.33\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/gobmk.pdf}
  \vspace{-0.6cm}
  \caption*{\scriptsize{Size (bytes)}}
  \vspace{-0.2cm}
  \caption{gobmk}
  \vspace{-0.2cm}
  \label{fig:gobmk}
  \end{subfigure}
  %\hspace{0.1cm}
  \begin{subfigure}[b]{0.33\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/mcf.pdf}
  \vspace{-0.6cm}
  \caption*{\scriptsize{Size (bytes)}}
  \vspace{-0.2cm}
  \caption{mcf}
  \vspace{-0.2cm}
  \label{fig:mcf}
  \end{subfigure}
  \begin{subfigure}[b]{0.33\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/sjeng.pdf}
  \vspace{-0.6cm}
  \caption*{\scriptsize{Size (bytes)}}
  \vspace{-0.2cm}
  \caption{sjeng}
  \vspace{-0.2cm}
  \label{fig:sjeng}
  \end{subfigure}
   \vspace{-0.3cm}
   \caption{Plots demonstrate the relationship between the compressed block size and reuse distance. Dark red circles correspond to the most frequent reuse distances for every size.} 
            %The first seven workloads ((a)--(g)) have some relation between the size and reuse, while the last two ((h)--(i)) do not show that size is indicative of reuse.}
   \vspace{-0.2cm}
\end{figure*}
Figures~\ref{fig:bzip2}--\ref{fig:sjeng} show the results of this experiment for nine
representative applications from our workload pool (our methodology is described in Section~\ref{sec:methodology}).
In seven of these applications (\emph{bzip2}, \emph{leslie3d},
\emph{gcc}, \emph{sphinx3}, \emph{tpch6}, \emph{soplex}), compressed
block size is an indicator of reuse distance (in other words, it can
be used to distinguish blocks with different reuse distances). In two
of the applications (\emph{mcf} and \emph{sjeng}), it is not. 
%: \emph{bzip2}, \emph{leslie3d}, \emph{gcc}, \emph{sphinx3}, \emph{tpch6},
%\emph{soplex}, \emph{mcf}, and \emph{sjeng} respectively. 
%We use the BDI~\cite{bdi} compression algorithm in this experiment.
Each graph is a scatter plot that shows the reuse distance distribution experienced by various compressed cache block sizes in these
applications.
Reuse distance is defined as the number of 
distinct addresses accessed between two consecutive accesses to the same address. 
There are nine possible compressed block sizes (based on the description from
the BDI work~\cite{bdi}). 
The size of each circle is proportional to the relative frequency of blocks of a particular size that exhibit
a specified reuse distance. Dark red circles indicate the most frequent reuse distances (up to three) for every size.

%For instance, in \emph{bzip2} (Figure~\ref{fig:bzip2}), 
%a large number of cache blocks are compressed to either 8, 36, or 64 (uncompressed) bytes and have a short reuse distance of less than 1000.
%In contrast, a significant number of blocks are 34 bytes and have a very large reuse distance of greater than 5000. 
%In \emph{sphinx3} (Figure~\ref{fig:sphinx3}), a significant number of blocks are compressed to 1-byte with long reuse distance of slightly more than 1000.

We can draw two major conclusions from these experiments.
First, there are many applications where block size is an indicator of reuse distance
(Figure~\ref{fig:bzip2}--\ref{fig:gobmk}). For instance, in
\emph{bzip2} (Figure~\ref{fig:bzip2}), a large number of cache blocks
are 8, 36, or 64 (uncompressed) bytes and have a short reuse distance
of less than 1000. In contrast, a significant number of blocks are 34
bytes and have a large reuse distance of greater than 5000. This
indicates that the 34-byte blocks can be deprioritized by the cache
when running \emph{bzip2} to improve performance. Similarly, in
\emph{sphinx3}, \emph{tpch6}, and \emph{soplex} (Figures~\ref{fig:sphinx3}--\ref{fig:soplex}), a significant number of
blocks are compressed to 1-byte with a long reuse distance of around 1000, 
whereas most of the blocks of other sizes have very short reuse distances of less than 100.
In general, we observe that data from 15 out of 23 of our evaluated applications show that block size is indicative of reuse.
This suggests that a compressed block size can be used as an indicator
of future block reuse which in turn can be used to prioritize the blocks of certain sizes (Section~\ref{sec:sip}),
improving application performance (see the effect on \emph{soplex} in Section~\ref{sec:single-core}).


%First, for many applications
%(e.g., Figure~\ref{fig:bzip2}--\ref{fig:gobmk}), there are certain
%frequent reuse distances that are specific for a single compressed size (or several sizes), while other applications (Figures~\ref{fig:mcf} and \ref{fig:sjeng}) have
%similar distributions of reuse distances within a size.
%For example, in \emph{gobmk} (Figure~\ref{fig:gobmk}) 1-byte blocks have a significant fraction
%of blocks with reuse distance more than 5000, and in \emph{soplex} (Figure~\ref{fig:soplex}) blocks of size 20
%have a signification fraction of blocks with short reuse. 
%In general, we observe that data from 14 out of 21 of our evaluated applications show that block size is indicative of reuse.
%This suggests that a compressed block size can potentially be used as an indicator
%of future block reuse which in turn can be used to prioritize the blocks of certain sizes (Section~\ref{sec:sip}),
%improving application performance (see the effect on \emph{soplex} in Section~\ref{sec:single-core}).


%Unlike the PC-based indicators~\cite{madcache,cachebasedonreusedist},
%the additional on-chip storage requirements to use such an indicator will be very modest, because the compressed cache block size
%is an integral part of the cache block tag~\cite{fpc,bdi,c-pack}

%The fact that there is likely a single dominant reuse distance associated with the most frequently occurring
%compressed cache block sizes indicates that compressed cache block size can be used to predict reuse characteristics
%of cache blocks. Unlike the PC-based solutions that predict reuse distance~\cite{madcache,cachebasedonreusedist},
%the additional on-chip storage requirements to predict the reuse will be very modest, because the compressed cache block size
%is an integral part of the cache block tag~\cite{fpc,bdi,c-pack}.

%Second, it is better to be sensitive to the compressed block size at a \emph{fine granularity}.
%Existing solutions~\cite{ecm} classify the blocks only at a coarser granularity (into \emph{big} or \emph{small} blocks) 
%and do not consider the potential relationship between size and reuse.
%In the case of \emph{bzip2} (Figure~\ref{fig:bzip2}), while 8 and 36-byte blocks have a short reuse distance, a significant
%fraction of cache blocks that get compressed to 34-bytes have a long reuse distance (between 5000 and 6000).
%In this case, attempting to use a coarse-grained classification to relate with reuse would end up associating
%the wrong reuse distance with either cache blocks of size 34-byte or 36-byte.
%To make things worse, the gap between some of the dominant cache block sizes for some applications (e.g., \emph{bzip2} and \emph{gcc}) is small (2--4 bytes).
%As a result, it is hard for a heuristic
%to predict a coarse-grained classification boundary with reasonable accuracy.

Second, there is usually no coarse-grained way to distinguish between block sizes
that are indicative of different reuse distances. In other words,
simply dividing the blocks into \emph{big} or \emph{small} blocks, as
recent work on compressed cache management does~\cite{ecm}, is not enough
to effectively identify the different reuse behavior of blocks of
different sizes; the distinction between block sizes should be done at
a finer granularity. This is evident for bzip2
(Figure~\ref{fig:bzip2}): while 8, 36, and 64-byte blocks have short
reuse distances, a significant fraction of the 34-byte blocks have
very long reuse distances (between 5000 and 6000). Hence, there is no
block size threshold that {\em divides/distinguishes} blocks with high
reuse and those with low reuse. Data from other applications (e.g.,
\emph{leslie3d}, \emph{gcc}, \emph{soplex}) similarly support this.

\REM{%%gpekhime: temporarily commented. DO NOT REMOVE
Figures~\ref{fig:reuse} and \ref{fig:leslie3d} show the results of this experiment for two 
representative applications from our workload pool, \emph{bzip2} and \emph{leslie3d}, respectively. 
The compressed cache design in this experiment uses the BDI~\cite{bdi} compression algorithm.  
Each graph is a scatter plot that shows the reuse distance distribution experienced by various 
compressed cache block sizes in these applications. 
Reuse distance is defined as the number of distinct addresses accessed between two consecutive accesses to the same address. There are nine possible compressed block sizes (based on the description from
the BDI paper~\cite{bdi}), and every size has blocks with different reuse distances. 
The size of each circle is proportional to the relative frequency of blocks of a particular size that exhibit 
a specified reuse distance. 
For instance, in \emph{bzip2}, a large number of cache blocks are compressed to either 8, 36, or 64 (uncompressed) bytes and have a short reuse distance of less than 1000.
In \emph{leslie3d}, a large number of blocks are compressed to 1-byte and have a reuse distance of less than 400 (short reuse). 

%Figure~\ref{fig:reuse} shows the results of this experiment for one 
%representative application from our workload pool, \emph{bzip2}, and a compressed cache design
%based on the BDI~\cite{bdi} compression algorithm.  
%The graph in this figure has nine possible compressed block sizes (based on the description from
%the BDI paper~\cite{bdi}), and every size can have blocks with different reuse distances. 
%In order to analyze both the reuse distance and the relative importance (frequency)
% of this distance, we use a scatter plot graph with larger circles for more frequent data points
%(the size of a circle is proportional to the relative frequency of a data point it represents).

\begin{figure*}[h!]
  \vspace{-0.2cm}
  \centering
  \begin{subfigure}[b]{0.49\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/bzip2.pdf}
  \caption*{\scriptsize{Size (bytes)}}
  \caption{bzip2 application.}
  %\vspace{-0.2cm}
  \label{fig:reuse}
  \end{subfigure}
  %\hspace{0.1cm}
  \begin{subfigure}[b]{0.49\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/leslie3d.pdf}
  \caption*{\scriptsize{Size (bytes)}}
  \caption{leslie3d application.}
  %\vspace{-0.2cm}
  \label{fig:leslie3d}
  \end{subfigure}
  \caption{Plots demonstrate the relationship between the compressed block size and reuse distance.}
  \vspace{-0.1cm}
\end{figure*}

We can draw two interesting conclusions from these experiments.
First, for many applications (e.g., Figure~\ref{fig:bzip2}--\ref{fig:gobmk}), there are certain 
frequent reuse distances that are specific for a single compressed size (or several sizes).
The fact that there is likely a single dominant reuse distance associated with the most frequently occurring 
compressed cache block sizes indicates that compressed cache block size can be used to predict reuse characteristics 
of cache blocks. Unlike the PC-based solutions that predict reuse distance~\cite{madcache,cachebasedonreusedist}, 
the additional on-chip storage requirements to predict the reuse will be very modest, because the compressed cache block size 
is an integral part of the cache block tag~\cite{fpc,bdi,c-pack}.

Second, it is best to learn the correlation between block size and reuse at a \emph{fine granularity}. 
Existing solutions~\cite{ecm} classify the blocks only at a coarser granularity (into \emph{big} or \emph{small} blocks) and do not consider the correlation between size and reuse.
In the case of \emph{bzip2}, while 8 and 36-byte blocks have a short reuse distance, a significant 
fraction of cache blocks that get compressed to 34-bytes have a long reuse distance (between 5000 and 6000). 
In this case, attempting to use a coarse-grained classification to correlate with reuse would end up associating 
the wrong reuse distance with either cache blocks of size 34-byte or 36-byte. 
Similar behavior can also be seen in the case of \emph{leslie3d} with 8-byte cache blocks 
(reuse distance closer to 1000) and 1, 24, 34, 36, and 40-byte blocks (with short reuse distance). 
To make things worse, the gap between some of the dominant cache block sizes is small (either 2 or 4-bytes).
As a result, it is hard for a heuristic 
to predict a coarse-grained classification boundary with reasonable accuracy.
}

\textbf{Code Example.}
The primary reason why this relationship exists is because in many applications, key data structures have
similar compression ratios and reuse patterns within a data structure, but different across
multiple different data structures. Figure~\ref{fig:example} demonstrates one simplified source 
code example based on the data structures observed in \emph{soplex}. It 
shows why the compressed size can be a good indicator of future reuse (as we observe
in Figure~\ref{fig:soplex}).\footnote{Note that our mechanisms are applicable to a variety of applications (Section~\ref{sec:results}) with
very different data structures and access patterns. The simplification in the example is done for clarity.}  

There are three data structures in this example: (i) array $A[N]$ of integer indexes that are smaller than
value $M$ (well-compressible with BDI~\cite{bdi} to 20-byte cache blocks), (ii) small
array $B[16]$ of floating point coefficients (incompressible, 64-byte cache blocks), and (iii) sparse matrix $C[M][N]$ with 
the main data (very compressible, 1-byte cache blocks). These data structures not only have different compressed block sizes, 
but also different reuse distances. Array $A[N]$ is accessed as $A[i]$ within the main loop, 
where $i$ changes every iteration of the outer loop,
and hence data is usually reused shortly (every iteration of the inner loop). This leads to a short reuse distance for 
the elements of this array. Accesses to array $B$ ($B[(i+j)\%16]$) lead to a short reuse distance
(usually every $16^{th}$ iteration of the inner loop). On the other hand, the reuse distance of array $C$ is data dependent on $A[i]$ -- it
is usually long and depends on what indexes are currently stored in array $A[i]$. 
Hence, this simplified example shows that {\em compressed
block size can indicate the reuse distance of a cache block}; a
1-byte block is likely to be reused much later than after it is
accessed, whereas a 20-byte block is likely to be reused very quickly.
If a cache
learns this relationship, it can prioritize 20-byte blocks over
1-byte blocks in its management policy. As we will show in
Section~\ref{sec:sip}, our compression-aware cache management policy
learns exactly this, leading to significant performance improvements
for \emph{soplex} (and other applications as shown in Section~\ref{sec:single-core}).


\lstdefinestyle{customc}{
  belowcaptionskip=1\baselineskip,
  breaklines=true,
  frame=L,
  xleftmargin=\parindent,
  language=C,
  showstringspaces=false,
  basicstyle=\footnotesize\ttfamily,
  keywordstyle=\bfseries\color{green!40!black},
  commentstyle=\itshape\color{purple!40!black},
  identifierstyle=\color{blue},
  stringstyle=\color{orange},
}

\lstdefinestyle{customasm}{
  belowcaptionskip=1\baselineskip,
  frame=L,
  xleftmargin=\parindent,
  language=[x86masm]Assembler,
  basicstyle=\footnotesize\ttfamily,
  commentstyle=\itshape\color{purple!40!black},
}

\lstset{escapechar=@,style=customc}
%\lstset{language=C,numbers=left,stepnumber=1,numbersep=3pt}
\begin{figure}[h!]
\vspace{-0.5cm}
\centering
\begin{lstlisting}
 int A[N];      // indexes (smaller than M): narrow values
 double B[16];  // coefficients: incompressible values
 double C[M][N];// sparse matrix: many zero values
 for (int i=0; i<N; i++) {
    for (int j=0; j<N; j++) {
      sum += B[(i+j)%16] * C[A[i]][j];
    }
 } 
\end{lstlisting}
\vspace{-0.4cm}
\caption{Code example: size and reuse distance relationship.}
\label{fig:example}
\vspace{-0.4cm}
\end{figure}

%In this example, the compressed size of 20 bytes usually indicates a short reuse distance. 
%A coarse-grain approach with a single threshold
%is \emph{ineffective} for this case (a case that is quite common based on our experiments), 
%because it cannot represent the \emph{fine-grain} correlation between the size and reuse (we have 20-byte blocks with short reuse distance 
%and 1-/64-byte blocks with long reuse distance). 
%This fine-grain relation between size and reuse can be exploited by a
%compression-aware cache management policy (see Section~\ref{sec:sip}) to improve application's performance (see Section~\ref{sec:single-core} for \emph{soplex}).

%\subsubsection*{Summary.} We make three key observations that motivate the need to consider cache block size while managing compressed caches:
%\begin{inparaenum}[(i)]
%\item considering cache block size along with temporal locality improves the effectiveness of replacement mechanisms in compressed caches,
%\item from an application perspective, each application has a number of sizes to which cache blocks get compressed, 
%with each application having its own set of dominant compressed block sizes, and
%\item compressed cache block size can be used to predict the future block reuse.
%\end{inparaenum}

%An enhancement to this mechanism is Dynamic RRIP (DRRIP) that uses set dueling~\cite{mlp} 
%to select the better performing of Static RRIP (described above) and Bimodal RRIP (BRRIP). 
%BRRIP is identical to SRRIP, 
%except it inserts blocks with a distant re-reference interval prediction with high probability 
%and inserts blocks with a long re-reference interval prediction with low probability.




==> camp/sections/2_motivation_old.tex <==
\section{Motivating Observations}
\label{sec:motivation}

%\begin{figure*}[!h]
%  \vspace{-0.4cm}
%  \centering
%  \includegraphics[width=0.90\textwidth]{figures/belady_example.pdf}
%  \caption{The downside of not including block size information in replacement decisions.}
%  \vspace{-0.2cm}
%  \label{fig:belady}
%\end{figure*}

Cache compression~\cite{fvc,fpc,bdi,iic-comp,c-pack} is a powerful mechanism that increases 
effective cache capacity and decreases off-chip bandwidth consumption. 
In this section, we show that cache compression adds an additional dimension
to cache management policy decisions -- \emph{the compressed block size} (or
simply \emph{the size}), which plays an important role in building more efficient management 
policies. We do this in three steps.

%Even with increased cache capacity, 
%efficient management of cached data is essential for maximizing performance. 
%In this section, it is first shown that 
%replacement decisions in compressed caches are improved by considering compressed cache block size along with temporal 
%locality to identify blocks to be evicted. Second, looking at cache compression reveals the challenges and opportunities involved in managing compressed caches.
%\REM{While
%these straightforward benefits of cache compression were studied in several
%recent works~\cite{bdi,c-pack,fpc}, very few works~\cite{ecm} look at the additional
%opportunities such as size-aware cache management policies created by cache compression.
%In this work, we show that cache compression adds an additional dimension
%to cache management policy decisions -- \emph{the compressed block size} (or
%simply \emph{the size}),
%that plays an important role in building more efficient management 
%policies. We do this in three steps. 
%}
%\textbf{Size matters.}
\subsection{Size Matters}
%\subsection{Impact of Cache Block Size on Replacement.}
%todo: add the footnote about MLP- unawareness
In compressed caches, replacement algorithms that take into account compressed cache block size along with locality to identify victim blocks can outperform existing policies that rely only on locality. 
In fact, Belady's optimal algorithm~\cite{belady} that relies only on locality (using perfect knowledge to evict the block that will be accessed furthest in the future) is sub-optimal in the context of compressed caches
with variable size cache blocks. 
Figure~\ref{fig:belady} demonstrates one possible example of such a scenario. In this figure, it is assumed that cache blocks are one of two sizes: 
\begin{inparaenum}[(i)]
\item uncompressed 64-byte blocks (blocks X and Y) and
\item compressed 32-byte blocks (blocks A, B, and C).
\end{inparaenum}
Initially (see \ding{202}), the 160-byte capacity cache contains four blocks: three compressed blocks (A, B, C) 
and one uncompressed block (Y). Consider the sequence of memory requests X, A, Y, B, and C (see  \ding{203}). In this case, after a request for X, Belady's algorithm (based on locality) will evict blocks B and C (to create 64-bytes of free space) that will be accessed furthest into the future. Over the next four accesses, this results in two misses (B and C) and two hits (A and Y). 

In contrast, a size-aware replacement policy can detect that it might be better to retain a set of smaller compressed cache blocks 
that receive more hits cumulatively than a single large (potentially uncompressed) cache block with better locality.
%The intuition is that multiple smaller blocks cumulatively can provide more hits than a single large cache block.
For the access pattern discussed above, a size-aware replacement policy makes the decision to retain B and C and evict Y to make space for X (see  \ding{204}). As a result, the cache experiences three hits (A, B, and C) and only one miss (Y) and hence outperforms Belady's optimal algorithm.\footnote{Note that if later (see  \ding{205}) there are three additional requests to blocks B, Y, and A (all three hits), the final
cache state becomes the same as the initial one. Hence, this example can represent steady 
state within a loop.} We conclude that using block size information in a compressed cache can lead to better replacement decisions. 
%~\footnote{In this paper, we assume that data is uncompressed in main memory.  Consequently, reducing miss rate results in a proportional reduction in memory bandwidth.  If, alternatively, compressed cache lines were stored in memory, 64 bytes of compressed data would be fetched under both policies in this example.  However, compression-aware replacement policies could yield {\em both} fewer misses and fewer bytes fetched than compression-oblivious policies in other situations.} 
%Note that if later (see  \ding{205}) there are three additional requests to blocks B, Y, and A (all three hits), the final
%cache state becomes the same as the initial one. Hence, this example can represent steady 
%state within a loop.  

\subsection{Size Varies}
Figure~\ref{fig:bdi} shows the distribution of compressed cache block 
sizes\footnote{Section~\ref{sec:methodology} describes the details of our evaluation 
methodology for this and other experiments.} for a set of representative workloads given a 2MB cache employing the BDI~\cite{bdi} cache compression algorithm 
(our results with FPC~\cite{fpc} compression algorithm show similar trends).  Even though the size of a compressed block is determined by the compression algorithm, 
under both designs, \textbf{compressed cache block sizes can vary significantly}, both 
\begin{inparaenum}[(i)]
\item within a single application (i.e., \emph{intra-application}) such as \emph{astar, povray}, and \emph{gcc} and
\item between applications (i.e., \emph{inter-application}) such as \emph{h264ref} and \emph{wrf}.
\end{inparaenum}

\begin{figure}[t]
  %\centering
  \centering
  \includegraphics[width=0.45\textwidth]{figures/distribution_bdi.pdf}
\caption{Compressed block size distribution for representative applications with the BDI compression algorithm.}
\vspace{-0.2cm}
\label{fig:bdi}
\end{figure}

\REM{
In order to show that compressed block sizes significantly vary both within 
and between
multiple applications, we conducted an experiment\footnote{Section~\ref{sec:methodology}
describes the details of our evaluation methodology for this and other experiments.} 
where we observed the cache block size distribution (collected from snapshots of the 2MB last-level-cache).
Figures~\ref{fig:bdi} and \ref{fig:fpc1} show the distributions of compressed block
sizes for a representative selection of applications from our workload pool.
In order to simplify both the data representation and analysis, we split
all possible sizes into 8-byte bins with one special bin for 64-byte (uncompressed)
blocks. 
We can draw two major conclusions from these figures.

First, the compressed block sizes vary significantly both 
(i) within an application (e.g., \emph{astar}), and
(ii) between the applications
(e.g., compare \emph{h264ref} and \emph{wrf}).
} 

Size variation within an application suggests that size-aware replacement policies could be effective for individual single-core workloads. 
Intra-application variation exists because applications have data that belongs
to different common patterns (e.g., zeros, repeated values, narrow values~\cite{bdi})
and as a result end up with a mix of compressed cache block sizes.
In the case of multiple cores with shared caches, inter-application variation suggests that even 
if an application has a single dominant compressed cache block size (e.g., \emph{lbm, h264ref} and \emph{wrf}), 
running these applications together will result in the shared cache experiencing a mix of compressed cache block sizes. 
Hence, size-aware management of compressed caches can be even more important for efficient cache utilization in multi-cores (as
we demonstrate quantitatively in Section~\ref{sec:multicore}).

\REM{
Inter-application variation suggests that
even if there is no significant variation within some individual applications, size
can vary significantly when these applications share the compressed cache (which creates
opportunities for size-aware replacement).
For example, if two (or more) applications have a dominant compressed block size
(e.g., \emph{h264ref} and \emph{wrf}), there is usually 
significant size variation (as with the variation within an application) 
when these applications are running together in a system
with a shared compressed cache.


Second, although the compressed block size is inherently dependent on
the compression algorithm that is used in cache compression,
comparison of the distributions from figure~\ref{fig:bdi} and figure~\ref{fig:fpc1} 
allows us to claim that size variation exists for different
compression algorithms: BDI~\cite{bdi} and FPC~\cite{fpc}. In general, we 
expect that our observations about the size variation hold for other 
compression algorithms as well, e.g., C-pack~\cite{c-pack}, and hence
we expect that the mechanisms we build based on these observations (see Section~\ref{sec:mve}) 
will be general
enough to work with different cache designs and compression algorithms.
}


\subsection{Size Indicates Reuse}
\label{sec:size-reuse}
%The benefits of knowing the size are not limited
%to providing an extra dimension that can be used in our replacement
%policies (Section~\ref{sec:mve}) either. 
We observe that elements belonging to the same data structure (within an application) sometimes compress to the same size.
This observation provides a new opportunity: using compressed size as an indicator of data reuse.
Typically an application's key data structures are accessed in a regular fashion, 
with each data structure having an identifiable access pattern~\cite{dataStructurePhase}. This regularity in accesses 
can be reflected in terms of predictable reuse distances of the cache blocks belonging to the data structures. 
Some prior works capture this by learning the relationship between the PC (instruction address) 
that accesses the data structure and the reuse distance~\cite{madcache,cachebasedonreusedist,singleUsage,DataCacheManagement}. 
%The key shortcoming of such solutions is the addition of new hardware to learn the correlation (if any) 
%between PC and reuse distance. 
On the other hand, if some key data structures have a dominant compressed size (i.e. a majority of the elements are compressed to one or few particular sizes), 
this size can be used as a signature for these data structures.
In such cases, regular access patterns to such data structures can be linked to (and hence be indicated by)
the compressed size of the cache blocks that store these data structures.
%. and hence predictable reuse 
%distances correlate with the compressed cache block size.
%Another key observation that we make is that a specific compressed block size
%within an application frequently correlates with a particular data structure,
%e.g., a certain array of elements stored in the compressed cache
%will likely have the same compressed block size
%for its data elements. This observation creates 
%an interesting opportunity. If an application's key data structures have
%certain dominant compressed sizes and these data structures
%also have some special properties when stored in the compressed cache, e.g.,
%certain average reuse distance,
%then compressed block size can be used as a predictor of these properties. 

To verify this, we conducted an experiment with our applications' memory traces
to look for the presence of a linkage between the compressed size and reuse.
For every block within an application, we computed the average distance (measured in memory requests) 
between the time this block was inserted into the compressed
cache and the time when it was reused next. We then accumulate this information
for all different sizes.
%We then average the reuse distance across the compressed
%blocks of the same size. 

\begin{figure*}[t]
  \vspace{-0.7cm}
  \centering
  \begin{subfigure}[b]{0.33\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/bzip2.pdf}
  \vspace{-0.6cm}
  \caption*{\scriptsize{Size (bytes)}}
  \vspace{-0.2cm}
  \caption{bzip2.}
  \label{fig:bzip2}
  \end{subfigure}
  %\hspace{0.1cm}
  \begin{subfigure}[b]{0.33\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/leslie3d.pdf}
  \vspace{-0.6cm}
  \caption*{\scriptsize{Size (bytes)}}
  \vspace{-0.2cm}
  \caption{leslie3d.}
  %\vspace{-0.2cm}
  \label{fig:leslie3d}
  \end{subfigure}
  \begin{subfigure}[b]{0.33\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/gcc.pdf}
  \vspace{-0.6cm}
  \caption*{\scriptsize{Size (bytes)}}
  \vspace{-0.2cm}
  \caption{gcc.}
  %\vspace{-0.2cm}
  \label{fig:gcc}
  \end{subfigure}
  %\vspace{-0.1cm}
  \begin{subfigure}[b]{0.33\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/sphinx3.pdf}
  \vspace{-0.6cm}
  \caption*{\scriptsize{Size (bytes)}}
  \vspace{-0.2cm}
  \caption{sphinx3.}
  %\vspace{-0.2cm}
  \label{fig:sphinx3}
  \end{subfigure}
  %\hspace{0.1cm}
  \begin{subfigure}[b]{0.33\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/tpch6.pdf}
  \vspace{-0.6cm}
  \caption*{\scriptsize{Size (bytes)}}
  \vspace{-0.2cm}
  \caption{tpch6.}
  %\vspace{-0.2cm}
  \label{fig:tpch6}
  \end{subfigure}
  \begin{subfigure}[b]{0.33\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/soplex.pdf}
  \vspace{-0.6cm}
  \caption*{\scriptsize{Size (bytes)}}
  \vspace{-0.2cm}
  \caption{soplex.}
  %\vspace{-0.2cm}
  \label{fig:soplex}
  \end{subfigure}
  \begin{subfigure}[b]{0.33\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/gobmk.pdf}
  \vspace{-0.6cm}
  \caption*{\scriptsize{Size (bytes)}}
  \vspace{-0.2cm}
  \caption{gobmk.}
  \vspace{-0.2cm}
  \label{fig:gobmk}
  \end{subfigure}
  %\hspace{0.1cm}
  \begin{subfigure}[b]{0.33\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/mcf.pdf}
  \vspace{-0.6cm}
  \caption*{\scriptsize{Size (bytes)}}
  \vspace{-0.2cm}
  \caption{mcf.}
  \vspace{-0.2cm}
  \label{fig:mcf}
  \end{subfigure}
  \begin{subfigure}[b]{0.33\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/sjeng.pdf}
  \vspace{-0.6cm}
  \caption*{\scriptsize{Size (bytes)}}
  \vspace{-0.2cm}
  \caption{sjeng.}
  \vspace{-0.2cm}
  \label{fig:sjeng}
  \end{subfigure}
   \vspace{-0.3cm}
   \caption{Plots demonstrate the relationship between the compressed block size and reuse distance. Red circles correspond to the most frequent reuse distances for every size. 
            The first seven workloads ((a)--(g)) have some relation between the size and reuse, while the last two ((h)--(i)) do not show that size is indicative of reuse.}
   \vspace{-0.2cm}
\end{figure*}
Figures~\ref{fig:bzip2}--\ref{fig:sjeng} show the results of this experiment for nine
representative applications from our workload pool (our methodology is described in Section~\ref{sec:methodology}): \emph{bzip2}, \emph{leslie3d}, \emph{gcc}, \emph{sphinx3}, \emph{tpch6},
\emph{soplex}, \emph{mcf}, and \emph{sjeng} respectively. We use the BDI~\cite{bdi} compression algorithm in this experiment.
Each graph is a scatter plot that shows the reuse distance distribution experienced by various compressed cache block sizes in these
applications.
Reuse distance is defined as the number of 
distinct addresses accessed between two consecutive accesses to the same address. 
There are nine possible compressed block sizes (based on the description from
the BDI work~\cite{bdi}). 
The size of each circle is proportional to the relative frequency of blocks of a particular size that exhibit
a specified reuse distance. Additional red circles indicate the most frequent reuse distances (up to three) for every size.
For instance, in \emph{bzip2} (Figure~\ref{fig:bzip2}), 
a large number of cache blocks are compressed to either 8, 36, or 64 (uncompressed) bytes and have a short reuse distance of less than 1000.
In \emph{sphinx3} (Figure~\ref{fig:sphinx3}), a significant number of blocks are compressed to 1-byte with long reuse distance of slightly more than 1000.

We can draw two conclusions from these experiments.
First, for many applications
(e.g., Figure~\ref{fig:bzip2}--\ref{fig:gobmk}), there are certain
frequent reuse distances that are specific for a single compressed size (or several sizes), while other applications (Figures~\ref{fig:mcf} and \ref{fig:sjeng}) have
similar distributions of reuse distances within a size.
For example, in \emph{gobmk} (Figure~\ref{fig:gobmk}) 1-byte blocks have a significant fraction
of blocks with reuse distance more than 5000, and in \emph{soplex} (Figure~\ref{fig:soplex}) blocks of size 20
have a signification fraction of blocks with short reuse. This suggests that a compressed block size can potentially be used as an indicator
of future block reuse which in turn can be used to prioritize the blocks of certain sizes (Section~\ref{sec:sip}),
improving application performance (see the effect on \emph{soplex} in Section~\ref{sec:single-core}).
%Unlike the PC-based indicators~\cite{madcache,cachebasedonreusedist},
%the additional on-chip storage requirements to use such an indicator will be very modest, because the compressed cache block size
%is an integral part of the cache block tag~\cite{fpc,bdi,c-pack}

%The fact that there is likely a single dominant reuse distance associated with the most frequently occurring
%compressed cache block sizes indicates that compressed cache block size can be used to predict reuse characteristics
%of cache blocks. Unlike the PC-based solutions that predict reuse distance~\cite{madcache,cachebasedonreusedist},
%the additional on-chip storage requirements to predict the reuse will be very modest, because the compressed cache block size
%is an integral part of the cache block tag~\cite{fpc,bdi,c-pack}.

Second, it is best to be sensitive to the compressed block size at a \emph{fine granularity}.
Existing solutions~\cite{ecm} classify the blocks only at a coarser granularity (into \emph{big} or \emph{small} blocks) 
and do not consider the potential relationship between size and reuse.
In the case of \emph{bzip2} (Figure~\ref{fig:bzip2}), while 8 and 36-byte blocks have a short reuse distance, a significant
fraction of cache blocks that get compressed to 34-bytes have a long reuse distance (between 5000 and 6000).
In this case, attempting to use a coarse-grained classification to relate with reuse would end up associating
the wrong reuse distance with either cache blocks of size 34-byte or 36-byte.
%Similar behavior can also be seen in the case of \emph{leslie3d}, \emph{soplex}, and \emph{gobmk} (Figures~\ref{fig:leslie3d}, \ref{fig:soplex}, and \ref{fig:gobmk} respectively).
%For example, for \emph{gobmk} 1-byte cache blocks and 40-byte blocks have a significant fraction long reuse distance blocks (around 1000),
%while 20-byte blocks has much shorter reuse distance (less than 100). This happens because different
%data types within this application have different compressed sizes.
To make things worse, the gap between some of the dominant cache block sizes for some applications (e.g., \emph{bzip2} and \emph{gcc}) is small (2--4 bytes).
As a result, it is hard for a heuristic
to predict a coarse-grained classification boundary with reasonable accuracy.

\REM{%%gpekhime: temporarily commented. DO NOT REMOVE
Figures~\ref{fig:reuse} and \ref{fig:leslie3d} show the results of this experiment for two 
representative applications from our workload pool, \emph{bzip2} and \emph{leslie3d}, respectively. 
The compressed cache design in this experiment uses the BDI~\cite{bdi} compression algorithm.  
Each graph is a scatter plot that shows the reuse distance distribution experienced by various 
compressed cache block sizes in these applications. 
Reuse distance is defined as the number of distinct addresses accessed between two consecutive accesses to the same address. There are nine possible compressed block sizes (based on the description from
the BDI paper~\cite{bdi}), and every size has blocks with different reuse distances. 
The size of each circle is proportional to the relative frequency of blocks of a particular size that exhibit 
a specified reuse distance. 
For instance, in \emph{bzip2}, a large number of cache blocks are compressed to either 8, 36, or 64 (uncompressed) bytes and have a short reuse distance of less than 1000.
In \emph{leslie3d}, a large number of blocks are compressed to 1-byte and have a reuse distance of less than 400 (short reuse). 

%Figure~\ref{fig:reuse} shows the results of this experiment for one 
%representative application from our workload pool, \emph{bzip2}, and a compressed cache design
%based on the BDI~\cite{bdi} compression algorithm.  
%The graph in this figure has nine possible compressed block sizes (based on the description from
%the BDI paper~\cite{bdi}), and every size can have blocks with different reuse distances. 
%In order to analyze both the reuse distance and the relative importance (frequency)
% of this distance, we use a scatter plot graph with larger circles for more frequent data points
%(the size of a circle is proportional to the relative frequency of a data point it represents).

\begin{figure*}[h!]
  \vspace{-0.2cm}
  \centering
  \begin{subfigure}[b]{0.49\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/bzip2.pdf}
  \caption*{\scriptsize{Size (bytes)}}
  \caption{bzip2 application.}
  %\vspace{-0.2cm}
  \label{fig:reuse}
  \end{subfigure}
  %\hspace{0.1cm}
  \begin{subfigure}[b]{0.49\linewidth}
  \centering
  \includegraphics[width=0.99\textwidth]{figures/leslie3d.pdf}
  \caption*{\scriptsize{Size (bytes)}}
  \caption{leslie3d application.}
  %\vspace{-0.2cm}
  \label{fig:leslie3d}
  \end{subfigure}
  \caption{Plots demonstrate the relationship between the compressed block size and reuse distance.}
  \vspace{-0.1cm}
\end{figure*}

We can draw two interesting conclusions from these experiments.
First, for many applications (e.g., Figure~\ref{fig:bzip2}--\ref{fig:gobmk}), there are certain 
frequent reuse distances that are specific for a single compressed size (or several sizes).
The fact that there is likely a single dominant reuse distance associated with the most frequently occurring 
compressed cache block sizes indicates that compressed cache block size can be used to predict reuse characteristics 
of cache blocks. Unlike the PC-based solutions that predict reuse distance~\cite{madcache,cachebasedonreusedist}, 
the additional on-chip storage requirements to predict the reuse will be very modest, because the compressed cache block size 
is an integral part of the cache block tag~\cite{fpc,bdi,c-pack}.

Second, it is best to learn the correlation between block size and reuse at a \emph{fine granularity}. 
Existing solutions~\cite{ecm} classify the blocks only at a coarser granularity (into \emph{big} or \emph{small} blocks) and do not consider the correlation between size and reuse.
In the case of \emph{bzip2}, while 8 and 36-byte blocks have a short reuse distance, a significant 
fraction of cache blocks that get compressed to 34-bytes have a long reuse distance (between 5000 and 6000). 
In this case, attempting to use a coarse-grained classification to correlate with reuse would end up associating 
the wrong reuse distance with either cache blocks of size 34-byte or 36-byte. 
Similar behavior can also be seen in the case of \emph{leslie3d} with 8-byte cache blocks 
(reuse distance closer to 1000) and 1, 24, 34, 36, and 40-byte blocks (with short reuse distance). 
To make things worse, the gap between some of the dominant cache block sizes is small (either 2 or 4-bytes).
As a result, it is hard for a heuristic 
to predict a coarse-grained classification boundary with reasonable accuracy.}

\subsubsection*{Why is Size Sometimes Indicative of Reuse?}
The primary reason why this relationship exists is because in many applications, key data structures have
similar compression ratios and reuse patterns within a data structure, but different across
multiple different data structures. Figure~\ref{fig:example} demonstrates one simplified source 
code example based on the data structures observed in \emph{soplex}. It 
shows why the compressed size can be a good indicator of future reuse (as we observe
in Figure~\ref{fig:soplex}).\footnote{Note that our mechanisms are applicable to a variety of applications (Section~\ref{sec:results}) with
very different data structures and access patterns. The simplification in the example is done for clarity.}  

There are three data structures in this example: (i) array $A[N]$ of integer indexes that are smaller than
value $M$ (well-compressible with BDI~\cite{bdi} to 20-byte cache blocks), (ii) small
array $B[16]$ of floating point coefficients (incompressible, 64-byte cache blocks), and (iii) sparse matrix $C[M][N]$ with 
the main data (very compressible, 1-byte cache blocks). These data structures not only have different compressed block sizes, 
but also different reuse distances. Array $A[N]$ is accessed as $A[j]$ within the main loop, 
where $j$ changes every iteration (in the inner loop),
and hence data is reused only between the iterations of the outer loop. This leads to a long reuse distance for 
the elements of this array. On the other hand, accesses to array $B$ ($B[(i+j)\%16]$) lead to a short reuse distance
(usually every $16^{th}$ iteration of the inner loop). The reuse distance of array $C$ is data dependent on $A[j]$ -- it
is usually long (but can also be short), depending on what indexes are currently stored in array $A[j]$. 

\lstdefinestyle{customc}{
  belowcaptionskip=1\baselineskip,
  breaklines=true,
  frame=L,
  xleftmargin=\parindent,
  language=C,
  showstringspaces=false,
  basicstyle=\footnotesize\ttfamily,
  keywordstyle=\bfseries\color{green!40!black},
  commentstyle=\itshape\color{purple!40!black},
  identifierstyle=\color{blue},
  stringstyle=\color{orange},
}

\lstdefinestyle{customasm}{
  belowcaptionskip=1\baselineskip,
  frame=L,
  xleftmargin=\parindent,
  language=[x86masm]Assembler,
  basicstyle=\footnotesize\ttfamily,
  commentstyle=\itshape\color{purple!40!black},
}

\lstset{escapechar=@,style=customc}
%\lstset{language=C,numbers=left,stepnumber=1,numbersep=3pt}
\begin{figure}[h!]
\vspace{-0.4cm}
\centering
\begin{lstlisting}
 int A[N];      // indexes (smaller than M): narrow values
 double B[16];  // coefficients: incompressible values
 double C[M][N];// sparse matrix: many zero values
 for (int i=0; i<N; i++) {
    for (int j=0; j<N; j++) {
      sum += B[(i+j)%16] * C[A[j]][i];
    }
 } 
\end{lstlisting}
\vspace{-0.2cm}
\caption{Code example: size and reuse distance correlation.}
\label{fig:example}
\vspace{-0.4cm}
\end{figure}

In this example, the compressed size of 20 bytes usually indicates a short reuse distance. 
A coarse-grain approach with a single threshold
is \emph{ineffective} for this case (a case that is quite common based on our experiments), 
because it cannot represent the \emph{fine-grain} correlation between the size and reuse (we have 20-byte blocks with short reuse distance 
and 1-/64-byte blocks with long reuse distance). 
This fine-grain relation between size and reuse can be exploited by a
compression-aware cache management policy (see Section~\ref{sec:sip}) to improve application's performance (see Section~\ref{sec:single-core} for \emph{soplex}).

%\subsubsection*{Summary.} We make three key observations that motivate the need to consider cache block size while managing compressed caches:
%\begin{inparaenum}[(i)]
%\item considering cache block size along with temporal locality improves the effectiveness of replacement mechanisms in compressed caches,
%\item from an application perspective, each application has a number of sizes to which cache blocks get compressed, 
%with each application having its own set of dominant compressed block sizes, and
%\item compressed cache block size can be used to predict the future block reuse.
%\end{inparaenum}

%An enhancement to this mechanism is Dynamic RRIP (DRRIP) that uses set dueling~\cite{mlp} 
%to select the better performing of Static RRIP (described above) and Bimodal RRIP (BRRIP). 
%BRRIP is identical to SRRIP, 
%except it inserts blocks with a distant re-reference interval prediction with high probability 
%and inserts blocks with a long re-reference interval prediction with low probability.




==> camp/sections/4_idea.tex <==
\section{CCM: Overview}
\label{sec:ideas}

Our proposed Compressed Cache Management (\carp) Policy consists of two
components: Minimal-Value Eviction (\mineviction{}) and Size-based Insertion
Policy (\insertionpolicy{}).  We explain the key ideas of each component in
this section and the implementation of each in the next section.  We also
propose Global \carp{} (or G-\carp), an adaptation of \carp{} for a cache with
a decoupled tag- and data-store and global replacement policy.

\subsection{Minimal-Value Eviction (\mineviction)} The key observation in
\mineviction{} is that evicting one or more important blocks of larger
compressed size may be more beneficial than evicting several more compressible,
less important blocks (see Section~\ref{sec:motivation}).  The idea behind
\mineviction{} is that each block has a value to the cache. This value is a
function of two key parameters: (i) the likelihood of future re-reference and
(ii) the compressed block size.  For a given  $<$prediction of re-reference,
compressed block size$>$ tuple, \mineviction{} associates \emph{a value to the
block}.  Intuitively, a block with higher likelihood of re-reference is more
valuable than a block with lower likelihood of re-reference and is assigned a
higher value.  Similarly, a more compressible block is more valuable than a
less compressible block because it takes up fewer segments in the data-store,
potentially allowing for the caching of additional useful blocks.  The block
with the least value in the cache is chosen as the next victim for replacement.

\subsection{Size-based Insertion Policy (\insertionpolicy)} The key observation
behind \insertionpolicy{} is that there is a correlation between cache block
reuse distance and compressed block size. \insertionpolicy{} exploits this
observation and inserts blocks of certain sizes with higher priority if doing
so reduces the cache miss rate.  \insertionpolicy{} is effective because there
is often a correlation between size and reuse distance either within an
application or within an application phase.  Altering the priority of blocks of
certain sizes with short or long reuse distances helps ensure more important
blocks stay in the cache.

At run-time, \insertionpolicy{} dynamically detects the set of sizes that, when
inserted with higher priority, reduce the number of misses relative to a
size-oblivious insertion policy.  \insertionpolicy{} uses a simple mechanism
based on dynamic set sampling~\cite{mlp} to make the prioritization decision
for various compressed sizes.

\subsection{\carp: Combining \mineviction{} and \insertionpolicy{}} Our final
mechanism, \carp, combines \mineviction{} and \insertionpolicy{} into one
comprehensive cache management policy for the compressed cache. To summarize,
\carp{} (i) changes the insertion priority of blocks with compressed sizes
determined to reduce the miss rate based on dynamically identified correlation
between block size and reuse distance, and (ii) evicts the set of blocks with
the least value based on a value function of block size and a prediction of
re-reference.

\subsection{Local vs. Global Insertion/Replacement} In addition to being an
effective mechanism for the traditional compressed cache with 
%a coupled tag- and data-store and 
local replacement policy, the key ideas behind \carp{} are even more effective
when applied to a cache with a decoupled tag- and data-store and global
replacement policy.  Towards this end, we propose Global \insertionpolicy{} (or
G-\insertionpolicy) and Global \mineviction{} (or G-\mineviction).  Together,
we combine these into Global \carp{} (or G-\carp).  For a traditional cache
structure, a local replacement policy considers only the blocks within a
\emph{single set} for candidates to replace.  The V-Way cache~\cite{v-way},
described in Section~\ref{sec:background}, with a decoupled tag- and data-store
allows for a global replacement decision where the pool of potential candidates
for replacement is much larger.  In Section~\ref{sec:results} we show that this
increases the effectiveness of our size-aware policies.


==> camp/sections/9_related.tex <==
\section{Related Work}

%\textbf{Size-Aware Replacement in On-Chip Caches}. We will provide comparisons to Baek et al's recently proposed Effective Capacity Maximizer (ECM) \cite{ecm}.
%Their mechanism employed a size-aware insertion and replacement policy for the on-chip compressed cache. 
%Unlike size-oblivious RRIP~\cite{RRIP} on which it is built, ECM inserts large blocks with lower priority than small blocks. 
%The threshold for what is considered a large block is determined dynamically at runtime using an equation derived from heuristics 
%and based on the current effective capacity and physical memory usage. During replacement, the largest block in the eviction pool is selected as the victim.

%This approach has several shortcomings and underperforms relative to our proposed mechanisms. 
%First, the threshold scheme is too coarse-grain. This is especially an issue in multi-core workloads 
%where a greater diversity of block sizes exists across workloads and a more intellgent replacement policy has much greater performance. 
%Second, ECM's mechanism does not consider the possibility of a correlation between block reuse and size. 
%Third, the insertion policy is not aggresive enough with deprioritizing the insertion of big blocks such that more important blocks can be prematurely evicted. 
%Fourth, this work does not consider a cache with a decoupled tag- and data-store where a size-aware replacement decision is even more beneficial. 
%TODO: describe all other problems: typos, tie to RRIP, ...

\textbf{Size-Aware Replacement in Web Caches}. Prior works in web caches have proposed many replacement strategies that consider object size, e.g. variable document size. 
ElAarag and Romano \cite{elaarag1, elaarag2} provide one of the most comprehensive surveys. 
While these proposed techniques serve much the same purpose as a replacement policy for an on-chip cache 
(e.g. making an informed decision on the optimal victim), they do so in a much different environment. 
Many proposed mechanisms rely on a recency list of all objects in the cache (e.g. \cite{size}) or consider frequency of object access (e.g. \cite{lru-sp}), 
which are extremely expensive techniques for an on-chip cache. 
In addition, many of these techniques try to maximize hit rate...instead of compressed objects with higher density of information (TODO).

Some prior works (e.g. \cite{luv, gd-size}) proposed function-based replacement policies that calculate the value of an object 
much like our proposed \mineviction{} policy. In particular, Bahn et al \cite{luv} proposed LUV where value of a block is computed 
as the division of rereference probability and the relative cost of fetching by size. 
Similar to other function-based techniques, however, these inputs cannot efficiently be computed or stored in hardware. 
Our proposed techique does not suffer from this problem and requires only simple parameters already built into on-chip caches.

%\textbf{V-Way}.
%The variable-way or V-Way~\cite{v-way} cache is a set associative cache with a decoupled tag- and data-store. 
%A defining characteristic is that there are more tag-entries than data-entries. 
%Forward and backward pointers are maintained in the tag- and data-store to link the entries. 
%This design allows associativity to effectively vary on a per-set basis by increasing the number of tag-store entries relative to data-store entries.
%Another benefit is the implementation of a global replacement policy, which is able to choose data-victims anywhere in the data-store. 
%This is in contrast to a traditional local replacement policy, which only considers data-store entries within a set as possible victims.

%The particular global replacement policy described in V-Way (called Reuse Replacement) consists of a reuse counter table (RCT) 
%with a counter for each data-store entry. Victim selection is done by starting at a pointer (PTR) to an entry in the RCT and searching for the first counter equal to zero, 
%decrementing each counter while searching and wrapping around if necessary. 
%A block is inserted with an RCT counter equal to zero and on a hit, the RCT counter for the block is incremented.

%\textbf{RRIP}.
%Re-Reference Interval Prediction (SRRIP) \cite{RRIP} uses an M-bit saturating counter per cache block as a Re-Reference Prediction Value (RRPV) 
%to predict the block's re-reference distance. Blocks are inserted with a long re-reference interval prediction (RRPV=$2^m-2$). 
%On a cache miss, the victim block is a block with a predicted distant re-reference interval (RRPV=$2^m-1$). 
%If there is no such block, the RRPV of all blocks is incremented by one and the process repeats until a victim is found. 
%On a cache hit, the RRPV of a block is set to zero (near-immediate rereference interval).

%An enhancement to this mechanism is Dynamic RRIP (DRRIP) that uses set dueling~\cite{setdueling} 
%to select the better performing of Static RRIP (described above) and Bimodal RRIP (BRRIP). BRRIP is identical to SRRIP, 
%except it inserts blocks with a distant re-reference interval prediction with high probability 
%and inserts blocks with a long re-reference interval prediction with low probability.

-compressed indirect index cache




==> chap10/9_results.tex <==


\section{Results}
\label{sec:results}
\subsection{Effect on DRAM Capacity}

Our LCP design aims to provide the benefit of increased effective main memory
capacity without making memory physically larger and without significantly
increasing the access latency. Figure~\ref{fig:capacity} compares the
compression ratio of LCP against that of other compression techniques: {\em i)}
Zero-Page compression, in which accesses to zero pages are served without any
cache/memory access (similar to LCP's zero page optimization), {\em ii)}
FPC~\cite{MMCompression}, {\em iii)} MXT~\cite{MXT}, and {\em iv)} Lempel-Ziv
(LZ)~\cite{lz}.\footnote{\small Our implementation of LZ performs compression at 4kB
  page-granularity and serves as an idealized upper boundary for the in-memory
  compression ratio. In contrast, MXT employs Lempel-Ziv at 1kB granularity.} We
evaluate the LCP framework in conjunction with two compression algorithms: BDI,
and BDI+FPC-fixed, in which each page can be encoded with either BDI or
FPC-fixed (Section~\ref{sec:design-prev-algos}).


%%% ONUR: Add citation or back-reference for the zero-page compression ONUR: MXT
%%% employs LZ? What is the difference between that and LZ? Unclear. In general,
%%% you have not described what these algorithms are.  ONUR: What is
%%% BDI+FPC-fixed. Please explain this (I tried above, but you cannot simply
%%% throw it at the reader...)


%Our LCP design aims to provide the benefit of increased effective DRAM capacity
%without making it phycially larger and without significant increase in access
%latency.  In order to evaluate the LCP's effectiveness in providing high
%effective compression ratio, we compare its compression ability (the effective
%compression ratio of the applications' memory footprints) with several prior
%DRAM designs (MXT~\cite{MXT}, FPC~\cite{MMCompression}), LZSS compression
%algorighm\footnote{LZSS compression is performed on the full 4-kB pages and
%serves as a practical boundary for the in-memory compression ratio.}~\cite{lz}
%and a simple compression design based on zero value pages.  We evaluate LCP
%framework with two compression techniques, namely BDI and BDI+FPC-fixed
%described in Section~\ref{sec:design}.


%%% ONUR: Why is MXT expected to do well. Justify. See my comment in parenthesis
%%% and fix it.  ONUR: ``Zero-Pages'' alone does not make sense. Can you rename
%%% this to ZPC (Zero Page Compression) both in text and figures...  ONUR:
%%% Please make the writing strong and explain things. Do not expect the reader
%%% to figure it all out.

We draw two conclusions from Figure~\ref{fig:capacity}. First, as expected, MXT,
which employs the complex LZ algorithm, has the highest average compression
ratio (2.30) of all practical designs and performs closely to our idealized LZ
implementation (2.60). At the same time, LCP (with either BDI or BDI+FPC-fixed)
provides a reasonably high compression ratio (up to 1.69 with BDI+FPC-fixed),
outperforming FPC (1.59).  Second, while the average compression ratio of
Zero-Page-Compression is relatively low (1.29), it greatly improves the
effective memory capacity for a number of applications (e.g., GemsFDFD, zeusmp,
and cactusADM) . This justifies our design decision of handling zero pages
specifically at TLB-entry level.
    
%Figure~\ref{fig:capacity} shows the results of this comparison.  First, as
%expected, MXT has the highest average compression ratio (2.30) of all practical
%designs and is close to the LZSS compression ratio (2.60). At the same time, LCP
%with both compression techniques provides reasonable compression ratio (up to
%1.69 with BDI+FPC-fixed), outperforming previously proposed DRAM compression
%design~\cite{MMCompression} based on FPC (1.59). 

%Second, noticable number of applications, e.g., GemsFDFD, zeusmp, and CactusADM,
%have significant number of zero pages (the average is 1.29), which justifies our
%design decision of handling zeros specifically at TBL-entry level.         

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.80\textwidth]{figures/Capacity.pdf}
  \caption{Effect of compression on main memory footprints.}
  \label{fig:capacity}
\end{figure}

\begin{figure*}[htb]
  \centering
  \includegraphics[width=0.99\textwidth]{figures/IPC.pdf}
  \caption{Performance comparison (IPC) of different compressed designs.}
  \label{fig:IPC}
\end{figure*}

\subsection{Effect on Performance}
\label{sec:results-perf}
Main memory compression can improve performance in two major ways: 1) reduced
memory footprint can reduce long-latency disk accesses, 2) reduced memory
bandwidth requirements can enable less contention on main memory bus, which is a
increasingly important bottleneck in systems. In our system performance
evaluations, we do not take into account the former benefit as we do not model
disk accesses (i.e., we assume that the uncompressed working set fits entirely
in memory). However, we do evaluate the performance improvement due to memory
bandwidth reduction (including our optimizations for compressing zero values
described in Section~\ref{sec:opt-zeros}). Evaluations using our LCP-framework
show that the performance gains due to the bandwidth reduction more than
compensate for the slight increase in memory access latency.

%This is in contrast to prior works~\cite{MXT,
%  MMCompression} that aimed only to minimize the performance loss due
%to compression.

%%% ONUR: I tried to fix the above, but there is still some redundancy. 

%%% ONUR: The last sentence: is it really correct? What is exactly in
%%% contrast to previous works? The result is contradictory, the
%%% evaluation is contradictory, or the previous work simply did not
%%% do this evaluation? You are not being clear here... I commented it
%%% out because I would be pretty annoyed as a reviewer if I saw such
%%% a sentence. Please either fix this or say none of it. 

%DRAM compression by itself cannot improve performance in our evaluations (we do
%not evaluate TLB miss latencies), but at the same time, it creates
%opportunities for bandwidth compression and avoids accesses to zero value pages
%and zero cache lines (see Section~\ref{sec:opt-zeros}). As a result, we aim
%to not only minimize performance losses due to increase in memory access
%latencies as in prior works~\cite{MXT, MMCompression}, but also improve
%performance, due to significant decrease in bandwidth consumption and in number
%of DRAM accesses.

In our experiments for both single-core and multi-core systems, we compare eight
different schemes that employ compression either in the last-level cache or main
memory or both. Table~\ref{table:schemes} describes the eight schemes.
\begin{table}[h!]\small
  \centering
  \begin{tabular}{|l|l|l|}
    \hline
    \textbf{No.} & \textbf{Label} & \textbf{Description}\\
    \hline
    1 & (None, None) & Baseline with no compression\\
    \hline
    2 & FPC-Cache & LLC compression using FPC~\cite{fpc}\\
    \hline
    3 & BDI-Cache & LLC compression using BDI~\cite{bdi}\\
    \hline
    4 & FPC-Memory & Main memory compression (Ekman and Stenstrom~\cite{MMCompression})\\
    \hline
    5 & LCP-BDI & LCP-framework with BDI\\
    \hline
    6 & (FPC, FPC) &  Designs 2 and 4 combined\\
    \hline
    7 & (BDI, LCP-BDI) &  Designs 3 and 5 combined\\
    \hline
    8 & (BDI, LCP-BDI+FPC-Fixed) & Design 3 combined with LCP-framework using BDI+FPC-Fixed\\
    \hline
  \end{tabular}
  \caption{List of evaluated designs.}
  \label{table:schemes}
\end{table}
\vspace{-0.3cm}
\subsubsection{Single-Core Results}

Figure~\ref{fig:IPC} shows the performance of single-core workloads using all
our evaluated designs normalized to the baseline (None, None). We draw three
major conclusions from the figure.


%Note that the (FPC, FPC) scheme has not been proposed before, but we evaluate it
%for completeness. 

%Figure~\ref{fig:IPC} shows the performance improvement of LCP-based designs
%(NoCompr-BDI, BDI-BDI, BDI-BDI+FPC-fixed) over the baseline design without
%compression, as well as comparison with two prior cache compression designs
%(BDI-NoCompr and FPC-Nocompr in our taxonomy, see
%Section~\ref{sec:design-taxonomy}), and two\footnote{We do not provide
%performance numbers for MXT, because its design requires 32MB L3 that operates
%on large 1kB blocks. Making MXT's last level cache comparable to other designs
%produces the unfairly low performance (DRAM accesses very expensive in MXT).  We
%believe that setting other designs with 1kB cache blocks also gives unfair
%advantage to MXT.} compressed DRAM designs (NoCompr-FPC, FPC-FPC). Note that
%FPC-FPC design never has been proposed before, but we evaluate it for
%completeness.

First, compared against an uncompressed system (None, None), the LCP design
using BDI compression (LCP-BDI) improves performance by 6.1\%.  This DRAM-only
compression scheme outperforms all LLC-only compression schemes and the
DRAM-only compression scheme proposed by Ekman and
Stenstrom~\cite{MMCompression} that uses the FPC algorithm (FPC-memory). We
conclude that our LCP framework is effective in improving performance by
compressing main memory.

%%% ONUR: Why is (None, FPC) not effective? What is going on in some benchmarks for this (astar, milc, omnetpp, xalancbmk)???

%the LCP-based baseline design (with
%BDI compression) is competitive against prior work proposals.

%We can draw two major conclusions. First, LCP baseline design (NoCompr - BDI)
%improves performance of the system with no compression (6.1\%), outperforming
%both the cache compression designs and the FPC-based compressed DRAM designs.
%This suggests that the LCP-based baseline design (with BDI compression) is
%competitive against prior work proposals. 

Second, the performance improvement of combined LLC and DRAM
compression is greater than that of LLC-only or DRAM-only compression
alone.  For example, LCP-BDI improves performance by 6.1\%,
whereas (BDI, LCP-BDI) improves performance by 9.5\%.  Intuitively, this
is due to the orthogonality of the benefits provided by cache
compression (retains more cache lines that otherwise would have been
evicted) and DRAM compression (brings in more cache lines that would
otherwise have required separate memory transfers on the main memory
bus). We will provide more analysis of this observation when analyzing
the effect on bandwidth in Section~\ref{sec:results-bandwidth}. We
conclude that our LCP framework integrates well with and complements
cache compression mechanisms.

%%% ONUR: You are not giving reasons. Just stating that something
%%% happens is not a good way of writing results. WHY does GemsFDTD's
%%% performance degrade with cache-only compression schemes?

%%% ONUR: Be consistent. cache-only --> LLC-only....

Third, a high compression ratio does not always imply an improvement
in performance. For example, while GemsFDTD is an application with a
highly compressible working set in both the cache and DRAM, its
performance does not improve with cache-only compression schemes (due
to the extra decompression latency), but improves significantly with
while significantly improving for DRAM-only compression schemes. In
contrast, cache-only compression is significantly beneficial for
omnetpp, whereas DRAM-only compression is not. This difference across
applications can be explained by the difference in their memory access
patterns. We observe that when temporal locality is critical for the
performance of an application (e.g., omnetpp and xalancbmk), then
cache compression schemes are typically more helpful. On the other
hand, when applications have high spatial locality and less temporal
locality (e.g., GemsFDTD has an overwhelming streaming access pattern
with little reuse), they benefit significantly from the bandwidth
compression provided by the LCP-based schemes. Hence, if the goal is to
improve performance of a wide variety of applications, that may have a
mix of temporal and spatial locality, our results suggest that
LCP-based designs with both DRAM and LLC compressed are the best
option. We conclude that combined LLC and DRAM compression that takes
advantage of our main memory compression framework benefits a wide
variety of applications.

%%% ONUR: I think the above explanation with temporal and spatial
%%% locality is not convincing. You need better explanations

%Third, even when applications have high effective compression ratio, e.g.,
%GemsFDTD, a compression design can not guarantee to have performance
%improvement. For example, BDI and FPC cache compression designs degrade
%performance of GemsFDFD (first and second bars), and, at the same time,
%DRAM-only compression designs improve performance significantly (third and
%fourth). On the other hand, cache compression significanly improves performance
%of omnetpp, but DRAM-only compression designs failed to do this (NoCompr-FPC
%even degrades it significantly). The main reason for such effects is the
%difference in types of locality that different applications might have. When the
%temporal locality is critical, then the cache compression designs are typically
%more helpful. On the other hand, when applications have high spatial locality,
%they can benefit more from the bandwidth compression provided by LCP-based
%designs. Hence, if the goal is to improve performance of the wide variety of
%applications, that have both local and spatial locality, our results suggest
%that LCP-based designs with both DRAM and LLC compressed are the best option.

%Second, performance improvement provided by DRAM-only and cache compression
%designs is noticably lower than that of joined designs, e.g., 9.5\% in BDI-BDI
%vs. 6.1\% in NoCompr-BDI.  Intuitively, this effect is mostly due to the
%orthogonality of the benefits provided by the cache compression (keeps more
%cache lines that otherwise could have been evicted), and DRAM compression
%(brings more cache lines that otherwise require separate memory transfers).  We
%will provide more analysis of this observation when analyzing the effect on
%bandwidth in Section~\ref{sec:results-bandwidth}

\vspace{-0.3cm}
\subsubsection{Multi-Core Results}

When the system has a single core, the memory bandwidth pressure may
not be large enough to take full advantage of bandwidth compression.
However, in a multi-core system where multiple applications are
running concurrently, savings in bandwidth (reduced number of memory
bus transfers) may significantly increase the overall system
performance.

%When only a single application is running in the system, the bandwidth pressure
%may not be significant enough to get the benefit from bandwidth compression.
%However, if multiple applications are running concurrently, sending multiple
%requests to DRAM at the same time, the decrease in number of transfers over the
%bus between LLC and DRAM becomes more critical to the overall system
%performance.


To study this effect, we conducted experiments using 100 randomly
generated multiprogrammed mixes of applications (for both 2-core and
4-core workloads). Our results show that bandwidth compression is
indeed more critical for multi-core workloads.  Using our LCP-based
design, LCP-BDI, the average performance
improvement\footnote{\small Normalized to the performance of the baseline
  system without any compression.} is 13.9\% for 2-core workloads and
10.7\% for 4-core workloads. We summarize our multi-core performance
results in Table~\ref{tbl:multicore}.

Figure~\ref{fig:many-core} shows the effect of varying the last-level
cache size on the performance benefit of our LCP-based design (using
BDI compression in main memory) both for single core and multi-core
systems across all evaluated workloads.  LCP-based designs outperform
the baseline across all evaluated systems, even when the L2 cache size
of the system is as large as 16MB. We conclude that our memory
compression framework is effective for a wide variety of core counts
and last-level cache sizes.


%% To study the effect of the LLC cache size on the performance of the LCP-based
%% designs for multicore architectures, we extended the initial experiment, and
%% evaluate the performance of LCP baseline design (None, BDI) with different L2
%% cache sizes (2M, 4M, 8M, 16M). Figure~\ref{fig:many-core} presents the result of
%% this experiment (every point is collected by averaging 100 randomly generated
%% mixes of applications).  We conclude that our mechanism is effective in
%% improving performance on a variety of multi-core systems and cache sizes.

%To study this effect, we conduct an experiment with 100 randomly generated mixes
%of applications (both for 2-core and 4-core workloads). Our results showed that
%bandwidth compression is indeed more critical for multicore workloads, with the
%average performance improvement\footnote{Normalized to the performance of the
%baseline system with no compression.} of 13.9\% for 2-core workloads, and 10.7\%
%for 4-core workloads (using LCP-based baseline design: NoCompr-BDI). We
%summarize our multicore performance results over the baseline without
%compression (2MB L2 cache) in Table~\ref{tbl:multicore}.

\begin{table}[ht]\small
  %\vspace{-0.2cm}
  \centering
  \begin{tabular}{cccc}
    \toprule
    \textbf{Cores}   &  \textbf{LCP-BDI} & \textbf{(BDI, LCP-BDI)} & \textbf{(BDI, LCP-BDI+FPC-fixed)} \\
    \midrule
    1  &  6.1\% &   9.5\% & 9.3\%  \\
    \cmidrule(rl){1-4}
    2 & 13.9\% & 23.7\% & 23.6\% \\
    \cmidrule(rl){1-4}
    4 & 10.7\%  & 22.6\% & 22.5\% \\
    \bottomrule
  \end{tabular}%
  \caption{Average performance improvement (weighted speedup) using LCP-based designs.}
  \label{tbl:multicore}%
\end{table}

\begin{figure*}[htb]
  \centering
  \begin{minipage}{5.0cm}
    \centering
    \includegraphics[height=3.0cm]{figures/1-core.pdf}\\
    a) 1-core
  \end{minipage}
  \begin{minipage}{5.0cm}
    \centering
    \includegraphics[height=3.0cm]{figures/2-core.pdf}\\
    b) 2-core
  \end{minipage}
  \begin{minipage}{5.0cm}
    \centering
    \includegraphics[height=3.0cm]{figures/4-core.pdf}\\
    c) 4-core
  \end{minipage}
  \caption{Effect of varying cache size on performance.}
  \label{fig:many-core}
\end{figure*}

%% \begin{figure}[htb]
%%   \begin{subfigure}{2.9cm}
%%     \centering
%%     \includegraphics[height=2cm]{figures/1-core.pdf}
%%     \caption{1-core}
%%     \label{fig:1-core}
%%   \end{subfigure}
%%   \begin{subfigure}{2.9cm}
%%     \centering
%%     \includegraphics[height=2cm]{figures/2-core.pdf}
%%     \caption{2-core}
%%     \label{fig:2-core}
%%   \end{subfigure}
%%   \begin{subfigure}{2.9cm}
%%     \centering
%%     \includegraphics[height=2cm]{figures/4-core.pdf}
%%     \caption{4-core}
%%     \label{fig:4-core}
%%   \end{subfigure}
%%   \caption{many-core}
%%   \label{fig:many-core}
%% \end{figure}

%% \begin{figure}[htb]
%%   \subfloat[1-core]{
%%     \label{fig:1-core}
%%     \centering
%%     \includegraphics[height=2cm]{figures/1-core.pdf}
%%   }
%%   \subfloat[2-core]{
%%     \label{fig:2-core}
%%     \centering
%%     \includegraphics[height=2cm]{figures/2-core.pdf}
%%   }
%%   \subf[4-core]{
%%     \label{fig:4-core}
%%     \centering
%%     \includegraphics[height=2cm]{figures/4-core.pdf}
%%   }
%%   \caption{many-core}
%%   \label{fig:many-core}
%% \end{figure}


%% \begin{figure}[htb]
%%   \begin{subfigure}[b]{0.16\textwidth}
%%     \includegraphics[width=0.99\textwidth]{figures/1-core.pdf}
%%     \caption{1-core}
%%     \label{fig:1-core}
%%   \end{subfigure}
%%   \begin{subfigure}[b]{0.16\textwidth}
%%     \includegraphics[width=0.99\textwidth]{figures/2-core.pdf}
%%     \caption{2-core}
%%     \label{fig:2-core}
%%   \end{subfigure}
%%   \begin{subfigure}[b]{0.16\textwidth}
%%     \includegraphics[width=0.99\textwidth]{figures/4-core.pdf}
%%     \caption{4-core}
%%     \label{fig:4-core}
%%   \end{subfigure}
%%   \caption{many-core}
%%   \label{fig:many-core}
%% \end{figure}


\begin{figure*}[htb]
  \centering
  \includegraphics[width=0.99\textwidth]{figures/Bandwidth.pdf}
  \caption{Effect of main memory compression on memory bandwidth.}
  \label{fig:bandwidth}
\end{figure*}
\begin{figure*}[htb]
  \centering
  \includegraphics[width=0.99\textwidth]{figures/Energy.pdf}
  \caption{Effect of main memory compression on power consumption of bus between
    memory controller and DRAM.}
  \label{fig:energy}
\end{figure*}


\subsection{Effect on Bus Bandwidth and Power}
\label{sec:results-bandwidth}

When DRAM pages are compressed, the traffic between the LLC and DRAM can also be
compressed. This can have multiple positive effects: {\em i)} reduction in the
average latency of memory accesses, which can lead to improvement in the overall
system performance, {\em ii)} decrease in the bus power consumption due to the
decrease in the number of transfers. 

%In a system, where DRAM pages are stored in the compressed form, there is an
%opportunity to compress the traffic between the LLC and DRAM. This can have
%multiple positive effects: 1) reduction in average latency of memory accesses,
%which can lead to improvement in the overall system performance, 2) decrease in
%the bus power consumption due to the decrease in the number of transfers. 

Figure~\ref{fig:bandwidth} shows the reduction in main memory
bandwidth between LLC and DRAM (in terms of bytes per kiloinstruction,
normalized to a system with no compression) using different
compression designs. Two major observations are in order.

%Figure~\ref{fig:bandwidth} shows the total reduction in bandwidth between LLC
%and DRAM (in terms of bytes per kilo instuction, normalized to the design with
%no compression) with different compression designs. We can draw three major
%conclusions from this figure.

First, DRAM compression schemes are more effective in reducing
bandwidth usage than cache compression schemes. This is because
cache-only compression schemes reduce bandwidth consumption by
reducing the number of LLC misses but they cannot reduce the bandwidth
required to transfer a cache line from main memory. Overall, combined
cache-DRAM compression schemes such as (FPC, FPC) and (BDI,
LCP-BDI+FPC-fixed) decrease bandwidth consumption by more than 46\% by
combining the reduction in both LLC misses and bandwidth required to
transfer each cache line.

%First, DRAM compression designs are more effective in compressing bandwidth than
%cache compression designs. This is because compression designs can only improve
%bandwidth indirectly by reducing the number of LLC misses.  Overall, FPC-FPC and
%BDI-BDI+FPC-fixed design can decrease bandwidth consumption by more than 46\%.

Second, there is a strong correlation between bandwidth compression
and performance improvement (Figure~\ref{fig:IPC}). Applications that
show a significant reduction in bandwidth consumption (e.g., GemsFDFD,
cactusADM, soplex, zeusmp, leslie3d, tpc*) also see large performance
improvements. There are some noticeable exceptions to this
observation, e.g., h264ref, wrf and bzip2. Although the memory bus
traffic is compressible in these applications, main memory bandwidth
is not the bottleneck for their performance.

%Second, there is a strong correlation between bandwidth compression and
%performance improvement (Figure~\ref{fig:IPC}).  Applications that have
%significant reduction in bandwidth consumption(GemsFDFD, cactusADM, soplex,
%zeusmp, leslie3d, tpc*) typically have significant improvement in performance as
%well. There are some noticable exclusions from this observation, e.g., h264ref,
%wrf and bzip2. The reason for this is that although their bus traffic is
%compressible, bandwidth is not the bottleneck for their performance.

\vspace{-0.3cm}
\subsubsection{Effect on Main Memory Bus Power}

By reducing the number of data transfers on the memory bus, a
compressed main memory design also reduces the power consumption of
the memory bus. Figure~\ref{fig:energy} shows the reduction in
consumed power\footnote{\small Normalized to the power of the baseline system
  with no compression.} by the main memory bus with different
compression designs. We observe that DRAM compression designs
outperform cache compression designs, and LCP-based designs provide
higher reductions than previous mechanisms for main memory
compression. The largest power reduction, 33\% on average, is achieved
by combined cache compression and LCP-based main memory compression
mechanisms, i.e. (BDI, LCP-BDI) and (BDI, LCP-BDI+FPC-fixed).  Even
though we do not evaluate full system power due to simulation
infrastructure limitations, such a large reduction in main memory bus
power consumption can have a significant impact on the overall
system's power, especially for memory-bandwidth-intensive
applications. We conclude that our framework for main memory
compression can enable significant memory power savings. 


%Positive effects of compression for bus are not limited to the decrease in
%bandwidth only.  Since the bus power consumption is proportional to the number
%of transfers~\cite{bus-energy}, it is possible to reduce it when the number of
%transfers is decreased.  [add reference on how critical is the power/energy of
%the bus?]

%Figure~\ref{fig:energy} shows the reduction in consumed
%power\footnote{Normalized to the power of the baseline system with no
%compression.} by the bus with different compression designs. We observe that
%DRAM compression designs outperfom cache compression designs, and LPC-based
%designs are better then corresponding FPC-based designs. The best power
%reduction is achieved by BDI-BDI and BDI-BDI+FPC-fixed designs (33\%). Such a
%reduction can have a noticable impact of the overall system's power, especially
%for bandwidth intensive applications, e.g., GemsFDFD. 


%sensitivity studies

\subsection{Analysis of LCP Structures and Parameters}
\vspace{-0.1cm}
\subsubsection{Effectiveness of the Metadata Cache} 
\label{sec:results-md}

The metadata (MD) cache is a critical structure in the LCP framework
as it helps the memory controller to avoid accesses to the LCP
metadata
(Section~\ref{sec:design-metadata-cache}). Figure~\ref{fig:mdcache}
shows the hit rate of a 512-entry (32kB) MD cache for an LCP design
that uses the BDI+FPC-fixed compression scheme for the single-core
system.\footnote{\small Other previously discussed designs have similar hit
  rate.} We draw two conclusions from the figure.

First, the average hit ratio is high (88\% on average), indicating
that the use of MD cache can significantly reduce the number of LCP
metadata accesses to main memory. This also justifies the absence of
significant performance degradation using the LCP framework
(Figure~\ref{fig:IPC}) even for applications that do not benefit from
compression. Second, some applications have significantly low MD cache
hit rate, especially, sjeng and astar. Analysis of the source code of
these applications revealed that accesses of these applications
exhibit very low locality. As a result, we also observed a low TLB hit
rate for these applications. Since TLB misses are costlier than MD
cache misses (former requires multiple memory accesses), the low MD
cache hit rate does not lead to significant performance degradation
for these applications.

%%% ONUR: Next version --> Need to provide performance sensitivity as
%%% you vary the size of this MC cache. 32kB is still large.


%% Metadata (MD) cache is the critical data structure in the LCP framework that
%% allows to avoid multiple access to DRAM in the common case of a hit to the LLC
%% (see Section~\ref{sec:design}.  Hence, the high hit rate of the MD cache is
%% crucial for LCP framework performance, since it avoids a significant increase in
%% DRAM access latency.

%% Figure~\ref{fig:mdcache} presents the hit rate of the MD cache for the LCP-based
%% design with DRAM compressed using BDI+FPC-fixed\footnote{Other previously
%%   discussed designs have similar hit rate.} and with TLB-ZeroBit optimization
%% (zero pages) disabled and enabled (first and second bar correspondingly). We can
%% draw two main conclusions from this figure.

%% First, the average hit ratio is high (90\% and 88\%) for both designs with small
%% 32kB MD cache, which suggests that it is effective in avoiding additional
%% accesses to DRAM (9 out of 10 cases on average). And, hence, this justifies the
%% absence of significant degradations for LCP-based designs in
%% Figure~\ref{fig:IPC} even when applications do not benefit from compression.

%% Second, several application have significantly lower hit ratio than the average,
%% most notably, sjeng and astar. Misses in the MD cache will increase the access
%% latencies for these applications, and can decrease performance in our
%% evaluations. At the same time, additional analysis of the applications' source
%% code, as well as TLB hit ratio analysis, show that the primary reason of this
%% effect is the random-access nature of most of the main memory accesses to the
%% key applications' data structures. Hence, we also observe low TLB miss rate for
%% these two applications.  TLB miss latency is at least an order of magnituge
%% higher~\cite{reference} than additional latencies that LCP-based system can
%% generate for these applications. So, we conclude that even in such uncommon
%% cases, MD low hit rate should not result in noticable performance degradations
%% on a real system.

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.89\textwidth]{figures/IndexCache.pdf}
  \caption{Effectiveness of the metadata cache.}
  \label{fig:mdcache}
\end{figure}
\vspace{-0.3cm}
\subsubsection{Analysis of Page Overflows}

As described in Section~\ref{sec:design-handling-overflows}, page
overflows can stall an application for a considerable duration. As we
mentioned in that section, we did not encounter any type-2 overflows
(the more severe type) in our simulations. Figure~\ref{fig:overflows}
shows the number of type-1 overflows per instruction. The y-axis uses
a log-scale as the number of overflows per instruction is very
small. As the figure shows, on average, less than one type-1 overflow
occurs every million instructions. Although such overflows are more
frequent for some applications (e.g., soplex and tpch2), our
evaluations show that this does not degrade performance in spite of
adding a 10000 cycle penalty for each type-1 page overflow. In fact,
these applications gain significant performance from our LCP
design. The main reason for this is that the benefits of bandwidth
reduction far outweighs the performance degradation due to type-1
overflows. We conclude that page overflows do not prevent the proposed
LCP framework from providing good overall performance.

%% Page size of overflow (increase over the current compressed page size limit) is
%% the most time consuming event that can be triggered in LCP framework.  As
%% described in Section~\ref{sec:methodology}, more common inner
%% overflows\footnote{As demonstrated in \cite{MMCompression} and in our own
%%   experiments, overflows over the uncompressed page size are orders of magnitude
%%   less frequent than inner overflows, so we united both of them in our results
%%   presentation for simplicity.} can take up to 10000 cycles, and this page is
%% locked during the required recompression. So, it is critical to show that such
%% events are rare in applications' execution.

%% Figure~\ref{fig:overflows} shows the number of overflows per committed
%% instruction, and since the numbers are relatively small, we put them in the
%% log-scale (the shorter the bar - the more frequent are page size overflows). As
%% we can see, the average number of overflows per instruction is less than
%% $10^{-6}$, which means a single overflow happens less than once per one million
%% instruction.  At the same time, there are few applications, e.g., soplex, that
%% have relatively high number of page size overflows, but our evaluations show
%% that it does significantly decrease performance of these few applications,
%% mostly because requests to other pages can still be serviced in parallel. We
%% conclude that page size overflows will typically not prevent LCP-based designs
%% from achieving good overall performance.

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.89\textwidth]{figures/Overflows.pdf}
  \caption{Type-1 page overflows for different applications.}
  \label{fig:overflows}
\end{figure}
\vspace{-0.3cm}
\subsubsection{Number of Exceptions}

The number of exceptions in the LCP framework is critical for two
reasons. First, it determines the size of the physical page required
to store the LCP. The higher the number of exceptions, the larger the
required physical page size. Second, it can affect an application's
performance as exceptions require three main memory accesses on an MD
cache miss (Section~\ref{sec:basic-mcf-overview}). We studied the
average number of exceptions (across all compressed pages) for each
application. Figure~\ref{fig:exceptions} shows the results of these
studies.

The number of exceptions varies from as low as 0.02/page for GemsFDTD
to as high as 29.2/page in milc (17.3/page on average). The average
number of exceptions has a visible impact on the compression ratio of
applications (Figure~\ref{fig:capacity}). An application with high
compression ratio also has relatively few exceptions per page. Note
that we do not restrict the number of exceptions in an LCP. As long as
an LCP fits into a physical page not larger than the uncompressed page
size (i.e., 4kB in our system), it will be stored in the compressed
form irrespective of how high the number of exceptions are. This is
why applications like milc have a large number of exceptions per
page. We note that etter performance is potentially achievable by
either statically or dynamically limiting the number of exceptions per
page, but a complete evaluation of the design space is a part of our
future work.

%% One of the critical parameters in the LCP page organization is the total number
%% of elements in the list of exceptions. This list defines a flexible part in the
%% compressed page organization, and for the best compressibility we would like to
%% keep it as small as possible. So, it is interesting to conduct an experiment
%% where the average number of exceptions per page is evaluated, and, hence,
%% indirectly see the effectiveness of our compression framework with the selected
%% compression algorithms.

%% Figure~\ref{fig:exceptions} presents the results of this experiment. As the
%% figure shows, the number of exceptions can vary significantly from as low as
%% 0.02 exceptions per page in GemsFDFD to as high as 29.2 in milc (average is
%% 17.3). These results reflects the effective compression ratios we observed in
%% Figure~\ref{fig:capacity}, typically application with high compression ratio has
%% relatively low number of exclusions.  One of the reasons why the number of
%% exceptions can be so high for some applications is that we do not restrict the
%% number of exceptions artificially in any way, so if the compressed page fits
%% into some permitted compressed page size, e.g., 512B or 4kB, then it would be
%% stored in the compressed form.

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.89\textwidth]{figures/Exclusions.pdf}
  \caption{Average number of exceptions per page for different applications}
  \label{fig:exceptions}
\end{figure}


\subsection{Comparison to Stride Prefetching}
\label{sec:results-prefetching-hints}

Our LCP-based framework improves performance due to its ability to
transfer multiple compressed cache lines using a single memory
request. Since this benefit resembles that of prefetching cache lines
into the last-level cache (LLC), we compare our LCP-based design to a
system that employs a stride
prefetcher~\cite{stride-prefetching}. Figures~\ref{fig:pref-ipc} and
\ref{fig:pref-bandwidth} compare the performance and bandwidth
consumption of three systems: 1)~one that employs stride prefetching,
2)~one that employs LCP, and 3)~one that employs LCP along with hints
from a prefetcher to avoid cache pollution
(Section~\ref{sec:opt-bandwidth}). Two conclusions are in order.

%%% ONUR: What isthe configuration of the prefetcher?

%%% ONUR: There is a lot of potential here... You can do very
%%% interesting research and write a great paper. All resonable
%%% systems employ prefetching, so exploring this interaction is
%%% critical.

%%% ONUR: I see Alaa's paper on prefetching + compression is not cited
%%% here. Any particular reason? Citing widely is important. It is a
%%% relevant paper. If you are stingy about citing, you will run into
%%% problems.

First, our LCP-based designs (second and third bars) outperform the
stride prefetcher for all but a few applications (e.g.,
libquantum). The primary reason for this is that a stride prefetcher
can considerably increase the memory bandwidth consumption of an
application due to inaccurate prefetch requests. On the other hand,
LCP obtains the benefits of prefetching without increasing (in fact,
while significantly reducing) memory bandwidth consumption.

Second, the effect of using prefetcher hints to avoid cache pollution
is not significant. The reason for this is that our systems employ a
large, highly-associative LLC (2MB 16-way) which is less susceptible
to cache pollution. Evicting the LRU lines from such a cache has
little effect on performance.

%% The primary reason for the performance improvements with LCP-based designs is
%% the ability to send multiple cache lines in one bus transfer.  This optimization
%% over the baseline LCP has positive effect on performance when there is enough
%% spatial locality in application's data accesses. There is a clear similarity in
%% exploiting this type of locality with bandwidth compression optimization and
%% stride prefetching~\cite{stride-prefetching}.  At the same, there is a
%% significant difference in how both techniques achieve their goals. While
%% prefetching typically trades decrease in LLC misses with bandwidth increase, our
%% bandwidth compression optimization achieves the decrease in LLC without
%% sacrificing bandwidth (and even improving it).  Hence, it is interesting to have
%% a comparison of the performance between stride
%% prefetching~\cite{stride-prefetching} and our design. We also looked at the
%% possibility of using existing hardware prefetchers as locality predictors to
%% avoid cache pollution.

%% %Prior work on cache compression and prefetching~\cite{compression-prefetching}.
%% Figure~\ref{fig:pref-ipc} and~\ref{fig:pref-bandwidth} shows the result of this
%% experiment.  We can draw two major conclusions from these results.

%% First, performance of the LCP-based BDI-BDI design (second bar) outperforms
%% stride prefetching on all but few applications (e.g., libquantum). The primary
%% reason for this is clear from Figure~\ref{fig:pref-bandwidth}, where for many
%% applications the bandwidth due to prefetching increases significantly, and,
%% hence, effects performance.

%% Second, using prefetching hints can help avoid cache pollution due to additional
%% cache lines LCP brings to the LLC, and we observe this effect in two
%% applications: GemsFDTD and soplex. But on average prefetching hints does not
%% have major effect on performance, mostly because our baseline 2MB 16-way L2
%% cache is not under enough pressure, so that evicting LRU cache lines has no
%% immediate effect on performance.

\begin{figure}[thb]
  \centering
  \includegraphics[width=0.89\textwidth]{figures/PrefetchIPC.pdf}
  \caption{Performance comparison with stride prefetching, and effect of using prefetcher
    hints with the LCP-framework.}
  \label{fig:pref-ipc}
\end{figure}

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.89\textwidth]{figures/PrefetchBandwidth.pdf}
  \caption{Bandwidth comparison with stride prefetching.}
  \label{fig:pref-bandwidth}
\end{figure}

\pagebreak
\subsection{Effect on GPU Systems}
\label{sec:gpu-bandwidth}

%%% ONUR: I do not get this. Are these results with the LCP framework
%%% or not... Writing is unclear. 

To show the general applicability of DRAM compression for different
architectures, we perform a preliminary experiment to analyze the
effect of main memory compression on memory bandwidth reduction for a
GPU architecture (AMD Evergreen ISA). Figure~\ref{fig:gpu-bandwidth}
shows the memory bandwidth reduction with three compression schemes:
1)~Frequent Pattern Compression, 2)~Base-Delta-Immediate Compression,
and 3)~Base-Delta-Immediate-rotate Compression (described in
Section~\ref{sec:design-prev-algos}). As the figure shows, all three
mechanisms significantly reduce the bandwidth requirements of most GPU
applications, with BDI-rotate showing the best results (48\% on
average). We conclude that our proposal is effective for GPU systems,
and can enable significant performance and energy-efficiency benefits
due to this reduction in main memory bandwidth especially in
memory-bandwidth-bound GPU applications.

%%% ONUR: Are all of the above three mechanisms *YOUR* LCP
%%% mechanisms???? Again, you need to be extremely clear if you are
%%% comparing to previous work or if you are evaluating your mechanism. 

%%% ONUR: This above section really needs a more detailed
%%% exploration. Please continue and you may find something evenn more
%%% exciting and novel.

\begin{figure}[!htb]
  \centering
  \includegraphics[width=0.89\textwidth]{figures/GPU-Bandwidth.pdf}
  \vspace{-0mm}
  \caption{Bandwidth Reduction in GPUs.}
  \label{fig:gpu-bandwidth}
\end{figure}




%%  shows that DRAM compression based on FPC,
%% BDI and especially BDI-rotate is effective in decreasing GPU's bandwidth
%% consumption (one of the main bottlenecks in GPU
%% performance~\cite{gpu-bandwidth}).  The decrease in bandwidth is quite
%% significant for most integer applications, e.g., FloydWarshall, with the best
%% average achieved by BDI-rotate (48\%).


==> chap1_alone.tex <==
\input{header}
\begin {document}

%% Double space document for easy review:
\renewcommand{\baselinestretch}{1.66}\normalsize
%\renewcommand{\baselinestretch}{1.2}\normalsize

\setcounter{chapter}{0}
\include{chap1}

\renewcommand{\baselinestretch}{1.0}\normalsize

\bibliographystyle{plain}
\bibliography{references}

\end{document}


==> chap2/software.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Software Interface}
\label{sec_software}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section we explore issues related to the design of a software
interface for FOO, we present a sample implementation of such an
interface, and we illustrate the use of this interface with several
examples.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{FOO Interface Design Issues}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Blah blah blah.  See Figure~\ref{recycled_while_loop}.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.

Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.

Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.

Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.

Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.

Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.
Blah blah blah blah blah blah blah blah.

\begin{figure}
    \singlespace
    \hrule
    \vspace{0.05in}
    \subfigure[A simple {\tt while} loop.]{
      \begin{minipage}{1.0in}
        \begin{smalltextcode}
          {\it/* Initialize y so that there is a RAW dependence} \\
          {\it \ * in iteration 6 of the loop: */} \\
          y[] = \{20, 21, 22, 23, 24, 25, {\bf 5}, \\
          \>\>    27, 28, 29, 30, ...\}; \\
          ... \\
          i = 0; \\
          while\ (++i < N) \{ \\
          \>  x[i] = x[y[i]]; \\
          \} \\
        \end{smalltextcode}
      \end{minipage}
      \begin{minipage}{1.0in}
        \includegraphics[height=1.4in]{chap2/graphs/while}
      \end{minipage}
      }
    \subfigure[Loop executed speculatively using recycled
    threads and dynamic scheduling.]{
      \begin{minipage}{1.0in}
        \begin{smalltextcode}
          \>  i = 0; \\
          \>  {\it /* Fork to all available processors: */} \\
          \>  fork\_threads(\&start); \\
          start: \\
          \>  {\it /* ++i is assumed to be atomic,} \\
          \>  {\it \ * my\_i is a local variable: */} \\
          \>  while\ ((my\_i = ++i) < N) \{ \\
          \>\>    begin\_speculation(my\_i); \\
          \>\>    x[my\_i] = x[y[my\_i]]; \\
          \>\>    end\_speculation(); \\
          \>\>    {\it/* speculation\_succeeded() doesn't return} \\
          \>\>    {\it \ * until this is the oldest epoch: */} \\
          \>\>    if(!speculation\_succeeded()) \{ \\
          \>\>\>      {\it /* Try again non-speculatively: */} \\
          \>\>\>      x[my\_i] = x[y[my\_i]]; \\
          \>\>    \} \\
          \>  \} \\
          \>  join\_threads(); \\
          \>  i = N; \\
        \end{smalltextcode}
      \end{minipage}
      \begin{minipage}{1.0in}
        \includegraphics[height=1.5in]{chap2/graphs/recycled}
      \end{minipage}
      }
    \hrule
    \caption{Speculative execution illustrated using a {\tt while} loop.}
    \label{recycled_while_loop}
\end{figure}

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> chap2_alone.tex <==
\input{header}
\begin {document}

%% Double space document for easy review:
\renewcommand{\baselinestretch}{1.66}\normalsize
%\renewcommand{\baselinestretch}{1.2}\normalsize

\setcounter{chapter}{1}
\include{chap2}

\renewcommand{\baselinestretch}{1.0}\normalsize

\bibliographystyle{plain}
\bibliography{references}

\end{document}


==> chap3_alone.tex <==
\input{header}
\begin {document}

%% Double space document for easy review:
\renewcommand{\baselinestretch}{1.66}\normalsize
%\renewcommand{\baselinestretch}{1.2}\normalsize

\setcounter{chapter}{2}
\include{chap3}

\renewcommand{\baselinestretch}{1.0}\normalsize

\bibliographystyle{plain}
\bibliography{references}

\end{document}


==> chap4/database.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Introduction}

Our goal is to parallelize individual transactions in a database,
using FOO.


==> chap4_alone.tex <==
\input{header}
\begin {document}

%% Double space document for easy review:
%\renewcommand{\baselinestretch}{1.66}\normalsize
\renewcommand{\baselinestretch}{1.2}\normalsize

\setcounter{chapter}{3}
\include{chap4}

\renewcommand{\baselinestretch}{1.0}\normalsize

\bibliographystyle{plain}
\bibliography{references}

\end{document}


==> chap5/conclusions.tex <==
This is the conclusion.  FOO rocks.

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "~/thesis/dissertation/main"
%%% End: 


==> chap5/lcp/sections/0_abstract.tex <==
\begin{abstract}

Data compression is a promising approach for meeting the increasing
memory capacity demands expected in future systems.  Unfortunately,
existing compression algorithms do not translate well when directly
applied to main memory because they require the memory controller to
perform non-trivial computation to locate a cache line within a
compressed memory page, thereby increasing access latency and
degrading system performance.  Prior proposals for addressing this
performance degradation problem are either costly or energy
inefficient.

  %% Main memory is a critical resource in modern systems. Future systems will
  %% require increasing amounts of main memory capacity to satisfy the needs of
  %% multiple applications concurrently running on multi-core processors as well as
  %% the large memory footprints of individual applications. However, simply adding
  %% more main memory to the system significantly increases both system cost and
  %% power consumption. One promising technique to address the main memory capacity
  %% problem is data compression. Unfortunately, directly applying previously
  %% proposed compression algorithms to main memory requires the memory controller
  %% to perform non-trivial computations to locate a cache line within the
  %% compressed main memory. These additional computations lead to significant
  %% increase in access latency, which can degrade system performance. Solutions
  %% proposed by prior work to address this performance degradation problem are
  %% either costly or energy inefficient.

By leveraging the key insight that all cache lines within a page
should be compressed to the same size, this paper proposes a new
approach \hfill to \hfill main \hfill memory \hfill 
compression---{\em Linearly \hfill Compressed} \\
{\em Pages}
(LCP)---that avoids the performance degradation problem without
requiring costly or energy-inefficient hardware.  We show that any
compression algorithm can be adapted to fit the requirements of LCP,
and we specifically adapt two previously-proposed compression
algorithms to LCP: Frequent Pattern Compression and
Base-Delta-Immediate Compression.

  %gpekhime: I removed this sentence, it is covered almost fully in the paragraph
  % anyway.
  %LCP greatly reduces the
  %amount of computation required to locate a cache line within the compressed
  %page, while keeping the hardware implementation of the proposed main memory
  %compression framework simple.

Evaluations using benchmarks from SPEC CPU2006 and five server
benchmarks show that our approach can significantly increase the
effective memory capacity (by 69\% on average). In addition to the
capacity gains, we evaluate the benefit of transferring consecutive
compressed cache lines between the memory controller and main
memory. Our new mechanism considerably reduces the memory bandwidth
requirements of most of the evaluated benchmarks (by 24\% on average),
and improves overall performance (by 6.1\%/13.9\%/10.7\% for
single-/two-/four-core workloads on average) compared to a baseline
system that does not employ main memory compression. LCP also
decreases energy consumed by the main memory subsystem (by 9.5\% on
average over the best prior mechanism).

  %gpekhime: To Vivek, please, have a look at the last sentence, maybe you have
  %some idea on how to make it "more fair".
\end{abstract}

%%   Main memory is a critical resource in modern systems, and it is
%% expected that future systems will require
%% increasing amounts of main memory in order to satisfy the needs
%% of multiple applications simultaneously running on many-core processors,
%% as well as the large memory footprint of each individual
%% application. A promising technique to address the DRAM capacity problem is
%% data compression. Unfortunately, directly applying well-known compression designs 
%% leads to either unacceptable increase in access latency (which in turn
%% can negatively affect performance) or severely increase hardware complexity and
%% energy efficiency.

%% In this paper, we propose a new main memory compression mechanism
%% that does not incur the latency penalty nor require power-hungry 
%% hardware. The key observation behind our proposal
%% is that if all the cache lines within a page are compressed to the
%% same size, then the location of a cache line in a compressed page 
%% does not require complex or/and inefficient address calculation.
%% Moreover, such a design will allow to retrieve multiple
%% consecutive cache lines for the cost of accessing
%% a single uncompressed cache line. 

%% Compared to prior main memory compression mechanisms, 
%% our studies show that our compressed DRAM design provides
%% significant increase in DRAM capacity and decrease in bandwidth consumption 
%% without significant increase in access latency and hardware complexity.
%% Our resultss show that this design can significantly increase the
%% main memory capacity (69 \%) using multiple compression algorithms 
%% (BDI~\cite{bdi} and FPC~\cite{fpc}). 
%% Moreover, we evaluate the benefits of transferring compressed cache
%% lines over the bus between DRAM and the memory controller
%% and show that it can considerably reduce bandwidth
%% and energy consumption of certain applications (32 \%), and
%% improve overall performance by 9.5\%.



==> chap5/lcp/sections/11_acknowledgements.tex <==
\section*{Acknowledgments}

%%% Onur: Let's make sure we acknowledge everyone who has provided
%%% good feedback individually.

Many thanks to Brian Hirano, Kayvon Fatahalian, David Hansquine and
Karin Strauss for their feedback during various stages of this
project.  We thank the anonymous reviewers and our shepherd Andreas Moshovos 
for their feedback.  We
acknowledge members of the SAFARI and LBA groups for their feedback
and for the stimulating research environment they provide. We
acknowledge the support of AMD, IBM, Intel, Oracle, Samsung and
Microsoft.  This research was partially supported by NSF (CCF-0953246,
CCF-1147397, CCF-1212962), Intel University Research Office Memory
Hierarchy Program, Intel Science and Technology Center for Cloud
Computing, Semiconductor Research Corporation and a Microsoft Research
Fellowship.


==> chap5/lcp/sections/6_integration.tex <==

\section{Integration with Compressed Last-Level Caches}
\label{sec:integration}
While our LCP-framework does not require any compression in the
last-level cache (LLC), it might be desirable to consider LLC
compression together with main memory compression for two
reasons. First, different applications may have different performance
bottlenecks, e.g., limited bandwidth or LLC capacity.  Hence,
compressing data at both levels of the memory hierarchy can improve
overall performance significantly by either improving an application's
cache hits or reducing its bandwidth requirements or both. Second, if
the same compression algorithm is employed to compress cache lines
both in LLC and in main memory, cache lines can be migrated between
the two levels without requiring any additional compression or
decompression, leading to significant improvements in energy
efficiency and latency. Our framework facilitates seamless integration
of LLC compression and main memory compression by ensuring that
compression algorithm is applied at the cache line granularity.

%%% ONUR: Are there any special benefits of the LCP framework that
%%% makes this integration easier? If so, write these down as that is
%%% important. I added the last sentence above but it needs teaking. 

To understand the benefits of integrating main memory compression with LLC
compression, we evaluate a set of designs where both LLC and main memory can be
either uncompressed or compressed with different compression mechanisms, e.g.,
BDI and FPC.  We present the results of these evaluations in
Section~\ref{sec:results-perf}.

%%%Table~\ref{table:taxonomy}
%%%shows the list of evaluated designs.

%%% ONUR: Give teh exact subsection where you present these if there
%%% is one (minor comment).


%% \begin{table}[!h]
%%   \centering
%%   \begin{tabular}{ll|ll}
%%     \toprule
%%     \textbf{LLC}   &  \textbf{DRAM} & \textbf{LLC} & \textbf{DRAM}  \\
%%     \toprule
%%     None  &  None &   BDI & None    \\
%%     \midrule
%%     FPC & None & None & BDI \\
%%     \midrule
%%     None & FPC & BDI & BDI \\
%%     \midrule
%%     FPC & FPC & BDI & BDI+FPC-fixed \\
%%     \bottomrule
%%   \end{tabular}
%%   \caption{List of Evaluated Compression Designs}
%%   \label{table:taxonomy}
%% \end{table}
%% \vspace{-0.5cm}

 
%All cache levels, except of L1, require the design similar to BDI and FPC
%compression mechanisms, where cache lines can be stored in both compressed and
%uncompressed form, and with additional tags available to benefit from
%compression.


%% \subsubsection{Compressed cache algorithms adoption and extension: BDI and FPC}
%% We have several requirements for the compression mechanisms that we allow to use
%% in our framework.  First, this algorithm should have efficient hardware
%% implementation with reasonable complexity (both compression and decompression).
%% Second, the decompression should be very fast (less than 10 cycles or better),
%% since it is on the critical part of the execution. Third, it should have fixed
%% compressed size to be applicable in our compressed page organization.

%% We found that several existing mechanisms (e.g., BDI~\cite{bdi} and
%% FPC~\cite{fpc}) satisfy or nearly satisfy our requirements. The BDI compression
%% has simple compression logic, very low decompression latency (1 cycle), and for
%% a fixed selection of base and $\Delta$ sizes it guarantees fixed compressed
%% size.  FPC has also simple compression logic, 5 cycle decompression latency,
%% but, unfortunately, it does not have fixed compressed size. To solve this
%% problem we adopt the FPC mechanism and introduce its variant called
%% \emph{FPC-fixed}.  We pick several fixed compressed sizes (16, 21, 32 and 44
%% bytes\footnote{Sizes are selected for the best integration with bandwidth
%%   compression.}) and after regular FPC compression, we check whether the
%% resulting compressed cache lines fits in the desired size limit. If yet, then
%% compression is successful, otherwise cache line is not compressible by
%% FPC-fixed.

%% Our framework requires all compressed cache lines to be the same size. In order
%% to achieve this during the initial page compression, multiple compression
%% algorithms are applied (BDI or/and FPC) with several fixed parameters, e.g.,
%% base - 4, $\Delta$ - 1 for BDI, or FPC-fixed with 32-byte limit. Then the
%% compression scheme with the smallest compression size is selected, and the
%% corresponding compressed page is store in the DRAM.

%% To improve the compression ratio of several floating point applications, e.g.,
%% leslie3d, we extend the baseline BDI mechanism to compress the data from some
%% floating point applications. The key observation is that in many cases floating
%% point values have the same exponent~\cite{IEEE standard} (8-12 bits), so this
%% can be exploited by using specific values of base and $\Delta$, e.g., base - 8,
%% $\Delta$ - 7. This extension does not require any changes in the BDI mechanism
%% itself, just one additional compressor unit should be added to perform the
%% initial compression.

%% The key part of our compressed main memory design is \textbf{compressed page
%%   organization}.  As we briefly described in Section~\ref{sec:basic}
%% (Figure~\ref{fig:page-organization}), every compressed page consist of three
%% distinct regions: (i) \emph{compressed data} region where every cache line on a
%% page is represented in the compressed form; (ii) \emph{metadata} region with the
%% information about every cache line compressilibility, as well, as pointers to
%% locations of non-compressed cache lines (exceptions); (iii) \emph{list of
%%   exceptions} that stores all cache lines that cannot be compressed with the
%% selected compression schemes in the uncompressed form.

%% Every cache line in the compressed data region has a fixed size slot, e.g., 16
%% byte for 64-byte cache line.  Fixed size requirement simplifies the offset
%% mapping between uncompressed and compressed pages. For example, if we need to
%% access the third 64-byte cache line within a page that was compressed with
%% factor 4 (from 64 to to 16 bytes), its offset on a page will change from $64
%% \times 2$ to $16 \times 2$.

%% It is not always possible to compress all cache lines within a page to a fixed
%% size slot. If a cache line cannot be compressed with the selected compression
%% algorithm, it is stored in the uncompressed form in the list of exceptions.  We
%% maintain a one byte slot with the metadata for every cache line within a
%% page. This slot stores a bit that indicates whether a particular cache line is
%% an exception or not, and a 6-bit index for a location inside the list of
%% exceptions (valid only for cache lines that are exceptions). The metadata region
%% consists of one-byte metada slots per cache line in the same order they are
%% stored in the compressed data section. In the case of 4kB page and 64-byte cache
%% lines, it is sufficient to allocate 64 bytes for all metadata on the page.

%% One of the primary advantages of storing the compressed data and metadata on the
%% same page is that it is then possible to avoid accesses to a different page to
%% get the metadata (costly row-for-miss accesses). Moreover, our page organization
%% allows to pipeline an access to the compressed data with an access to the
%% corresponding metadata (these accesses are independent, so an access to the
%% compressed data can be done speculatively). This effectively avoids accesses
%% serialization and, hence, signigicant increase in access latency does not
%% happen.


%% Note that the proposed page organization allows to win in capacity only for the
%% pages for which the compression factor is high enough not only to provide the
%% space for the metadata and list of exceptions, but also to leave significant
%% space that can be used by operating system to allocate other pages. For example,
%% 4kB page, compressed with factor 4 and 10 exceptions, will fit in a 2kB space,
%% so the other 2kB can be used for another page with similar space requirement
%% (see Section~\ref{sec:design-os} for details).

 
%% \textbf{Page table entry extension.}  To distinguish between compressed and
%% uncompressed pages both hardware and operating system require information
%% about pages' compressibility. Moreover, a complete knowledge about page
%% compression encoding used, e.g., BDI with compression ratio 4, is needed to
%% perform compression/decompression between main memory (DRAM) and last level
%% cache.  To achieve this we propose to add \ctype, \csize and \cbase bits to
%% the page table entries maintained by operating system. The corresponding
%% change should be also made either to the existing TLB (translation lookaside
%% buffer) entry or can be stored in a separate hardware data structure.



%% \subsection{Main Memory Compression in Action}
%% We now describe the operation flow of our main memory compression framework in
%% more details, assuming that only main memory is compressed.

%% First, when the memory request is coming from the CPU, and the corresponding
%% page is not currently in the DRAM, this request is transferred to the disk,
%% which stores data in the uncompressed form.  On the first access to a page, the
%% data is then accessed from the disk and compressed using several compression
%% algorithms supported by our compression framework.  Then, the compressed page
%% with the smallest size is selected to be stored in the DRAM.  After this, the
%% data is transferred in the compressed form over the bus to the memory controller
%% (MC), where it is decompressed.  Uncompressed data is then stored in the caches
%% and transferred to the CPU.

%% If later the same compressed page is accessed from DRAM, there are two main
%% scenarios to consider based on the request type: read or write.  In the case of
%% a read request, there are two possible cases: the required cache line is either
%% compressed, then it is simply accessed from the compressed data region, or
%% uncompressed, then an additional access is performed to obtain the cache line
%% from the list of exceptions (based on the \eindex stored in the metadata).

%% In the case of a write request, there are two main cases to consider as well.
%% First, if a stored cache line does not increase the total page size, so that the
%% page still fits in the allocated space by OS (no overflow), then the data is
%% simply written to the corresponding compressed data slot, and, the list of
%% exceptions and the metadata are updated accordingly (if needed).  For example,
%% previously non-compressed cache line (exception) when replaced with the zero
%% cache line requires the metadata update: \zbit, \ebit and \eindex are updated.
%% Second, if after the write the compressed page does not fit in the allocated
%% space (overflow), this page is locked for any accesses.  This page is then
%% either reallocated to a pool with larger pages by OS, or decompressed to be
%% stored in the uncompressed form. The latter happens if the page does not fit in
%% the maximum page size, e.g., 4kB.


%% \subsubsection{Memory Controller Operation}

%% The memory page organization we described previously, is effective in pipelining
%% the requests to the metadata and compressed data. But it still increases the
%% latency of an access, because both requests to the same page cannot fully
%% overlap[more details?], and increases DRAM bandwidth consumption. To avoid these
%% negative effects, we propose to use a small 512-entry \emph{index cache} [maybe,
%%   metadata cache] located in the MC that caches compressed pages' metadata.

%% The main benefit of implementing such a cache is that for a commonly accessed
%% page it avoids an additional DRAM access to get the compressed page
%% metadata. This allows to perform two optimizations in the baseline page
%% organization flow.  First, if the metadata of the page is known before the
%% access (index cache hit), then, for a requested cache line, we know whether it
%% is compressed (based on \ebit) or in the list of exceptions.  If it is the list
%% of exceptions, we have cache line's \eindex that can be used to access the data.
%% In both cases, MC needs to issue only a single memory request to the compressed
%% page. Hence, we avoid significant latency and bandwidth consumption increase.
%% Second, in a case of a hit, we also get the cache line's \zbit, and when it is
%% set, MC can fully avoid memory request by simply returning zero cache line. This
%% allows to win both in latency and in bandwidth consumption over the baseline
%% organization.

%% The key in the index cache efficiency is that it can deliver high average hit
%% ratio (more than 90\% on average, see Section~\ref{sec:results}), while using
%% only the storage of 32kB (512 entries, 64 bytes each). Note that the
%% implementation of this cache is not mandatory for our framework, it is just an
%% optimization that significantly improves performance and decreases bandwidth
%% consumption.

%% One of the additional advantages of main memory compression is the potential of
%% decreasing bandwidth consumption, and, as a result, decreasing the power
%% consumed by the bus between the main memory and the LLC.  Modern implementations
%% of the DRAM-based main memory are typically highly optimized for accessing
%% sequential chunks of data (usually, a cache line size of $\cls$ bytes).  In our
%% design the compressed data is located sequentially in the compressed data region
%% and its size is known. Hence, when a regular access to DRAM is serviced, the
%% memory controller (MC) receives $\cls$ bytes of data from DRAM that starts with
%% $\ccls$ of requested cache line, and then ends up with $\cls$ - $\ccls$ bytes
%% from one or multiple adjacent cache lines.  Based on the compressed page type
%% $\ctype$, MC can determine how many adjacent cache lines are available after the
%% request was serviced.  For example, if 1) the compression has factor 4, 2)
%% originally requested cache line has $\ebit$ not set, and 3) two adjacent cache
%% lines have \ebit not set as well, then, three compressed cache lines are
%% available in the MC after the servicing just one request.  It is then possible
%% to decompress these additional cache lines as well, and put them in the LLC (if
%% they are not there already).

%% If these cache lines are later requested by the CPU (before eviction), then
%% costly LLC misses are avoided, which means improved performance and decrease in
%% bandwidth consumption and power consumed by the bus.  The effect of bandwidth
%% compression is significant for the performance of applications with high spatial
%% locality and high bandwidth traffic between LLC and DRAM.  At the same time,
%% bringing multiple additional cache lines to the LLC might pollute the cache by
%% evicting other useful cache lines.

%% We consider two solutions to this problem.
%% %cache lines should be put in the LLC, since they can evict useful data that is already there.
%% The first simple solution is to add all available cache lines. This results in
%% eviction of some other cache lines, but there is a high probability that these
%% cache lines belongs to non-frequently used data (we assume LRU replacement
%% policy).  A more sophisticated solution is to predict additional cache lines'
%% usefulness based on applications' accesses locality.  One way of achieving this
%% is by using hints from the existing stride prefetchers~\cite{stride-prefetching}
%% hardware.  Prefetchers may suggest which adjacent cache lines are useful in the
%% nearest future.  This solution can potentially help to avoid cache pollution (if
%% any).  Both solutions were evaluated in Section~\ref{sec:results-prefetch}.

%% Note that bandwidth compression as proposed does not require any changes in the
%% DRAM or compressed page organization. Only memory controller logic has to be
%% changed to determine the number of available cache lines in the serviced
%% request.


==> chap5/lcp/sections/7_related.tex <==
\section{Related Work}
\label{sec:relatedwork}
%bandwidth compression
Previous work looked at possibility of bandwidth compression~\cite{register-caching,fvc-bus,LinkCompression}
between LLC and DRAM. While significant potential decreases in bandwidth consumption are reported,
none of the work looked at the possibility of compressing bandwidth without increase in latency 
(that is due the presence of compressors/decompressors, located on both ends of the memory bus).


==> chap5/lcp/sections/temp.tex <==
As we briefly mentioned before, one of the additional advantages of main memory
compression is the potential of decreasing bandwidth consumption, and, as a result, 
to decrease the power consumed by the bus between the main memory and the LLC. 
Modern implementations of the DRAM used for main memory are typically
highly optimized for accessing sequential chuncks of data (usually cache line size of $\cls$ bytes). 
Fortunately, in our design the compressed data is located sequentially in the compressed data region, 
and, hence, when a regular access to DRAM is serviced, the memory controller (MC) receives $\cls$ bytes 
of data from DRAM that starts with the requested cache line. Based on the compressed page type $\ctype$, MC can
determine how many more adjacent cache lines are available after this request was serviced. For example,
if 1) the compression has factor 4, 2) originally requested cache line has e-bit not set, and
3) two adjacent cache lines have e-bit not set as well, three compressed cache lines are available
in the MC instead of just one. 
It is then possible to decompress these additional cache lines as well, and put them in the LLC (if they
are not there already).


If these additional cache lines are later requested by the CPU, then a potentially costly LLC miss is
avoided, and, hence, access latency decreases, as well as bandwidth consumption and energy of the bus.
This can significantly increase the performance of some applications, especially those that have high
spatial locality and high bandwidth traffic between LLC and DRAM. At the same time, bringing multiple 
additional cache lines raises up the question of whether all, only selected, or none of these additional
cache lines should be put in the LLC, since they can evict useful data that is already there.
The simple solution is to add all possible cache lines, because even if they evict something from the cache,
this is probably non-frequently used data (we assume LRU replacement policy). A more sophisticated
option is to predict additional cache line usefulness based on applications' accesses locality.
One way of achieving this is by using hints from the existing hardware stride prefetchers~\cite{stride-prefetching} 
that can suggest whether adjacent cache lines are useful in the nearest future. This solution
can potentially help to avoid cache pollution. We evaluated both options in Section~\sec{sec:results-prefetch}.


Bandwidth compression as proposed does not require any changes in the DRAM or compressed page organization, only
memory controller logic has to be changed to determine the number of available cache lines in the serviced request.


  


==> chap5_alone.tex <==
\input{header}
\begin {document}

%% Double space document for easy review:
\renewcommand{\baselinestretch}{1.66}\normalsize
%\renewcommand{\baselinestretch}{1.2}\normalsize

\setcounter{chapter}{4}
\include{chap5}

\renewcommand{\baselinestretch}{1.0}\normalsize

\bibliographystyle{plain}
\bibliography{references}

\end{document}


==> chap6.tex <==
\chapter{Flexible and Efficient Bandwidth Compression for GPUs}
\input{caba/sections/1_introduction}
\input{caba/sections/2_motivation}
\input{caba/sections/3_CABA_1}
%\input{sections/3_CABA_2}
%\input{sections/3_CABA_3}
\input{caba/sections/4_compression_1}
%\input{sections/4_compression_2}
%\input{sections/4_compression_3}
\input{caba/sections/5_methodology}
\input{caba/sections/6_results}
%\input{sections/7_applications}
\input{caba/sections/8_related}
\input{caba/sections/9_conclusion}
%


==> code-macros.tex <==
%% The Code environment %%%

%% The following commands are so we can automatically number and symbolically reference
%% lines.
%% The ``codelinenumber'' counter counts the current line number
\newcounter{codelinenumber}
%% The \zeroli command zeros the line number counter
\newcommand{\zeroli}{\setcounter{codelinenumber}0}
%% The \li command bumps the counter, outputs it, and skips some space
%% It also GLOBALLY sets the value of \@currentlabel, so that the \label
%% commands on the same line work OK.  The problem otherwise is that Latex
%% uses groups on each field of a line in tabbing mode, and this causes
%% \@currentlabel to get reset as soon as a field ends (e.g. at the \').
%% Now, the label can appear after the \\, as in
%%	\li \>\>$x\gets y$ \\ \label{li:assign-x}
%%

\makeatletter
\def\@startline{\global\@curtabmar\@nxttabmar\relax
   \global\@curtab\@curtabmar\setbox\@curline\hbox
    {}\@startfield\global\lifalse\strut}

\newenvironment{code}{%
\setbox\strutbox\hbox{\vrule height 9pt depth 4pt width0pt}%
\noindent\begin{tabbing}%
\zeroli\setlength{\tabbingsep}{1em}
\hspace*{1em}\=999\ifdoubledigit9\fi
\=\ {\bf if} \={\bf then} \={\bf if} \={\bf then}
	\={\bf if} \={\bf then} \={\bf if} \={\bf then} \={\bf if} \={\bf then}
	\={\bf if} \=\+\+\kill}{\end{tabbing}}

\newif\ifdoubledigit
\newcommand{\codebox}[1]{\setbox0=\vbox{\begin{code}#1\end{code}}
\ifnum\c@codelinenumber>9\global\doubledigittrue\else\doubledigitfalse\fi
\vskip1sp\noindent\hskip-14pt%% 
\parbox{\textwidth}{\begin{code}\protect#1\end{code}}\global\let\@currentlabel=\thesection}

\newif\ifli
\newcommand{\li}{\global\litrue\stepcounter{codelinenumber}%
\ifdoubledigit%
\hbox to8pt{\hss\thecodelinenumber\hskip5pt}\else%
\hbox to8pt{\hskip-1pt\thecodelinenumber\hss}\fi%
\xdef\@currentlabel{\p@codelinenumber\thecodelinenumber}\'}
\makeatother

\newcommand{\For}{{\bf for} }
\newcommand{\To}{{\bf to} }
\newcommand{\By}{{\bf by} }
\newcommand{\Downto}{{\bf downto} }
\newcommand{\While}{{\bf while} }
\newcommand{\Repeat}{\>\>{\bf repeat}\'}
\newcommand{\Until}{\>\>{\bf until}\'}
\newcommand{\If}{{\bf if} }
\newcommand{\Then}{\>{\bf then}\>}
\newcommand{\Else}{\>{\bf else}\>}
\newcommand{\ElseIf}{{\bf elseif} }
\newcommand{\ElseNoIf}{{\bf else} }
\newcommand{\Do}{\>\>{\bf do}\'}
\newcommand{\Return}{{\bf return} }
\newcommand{\Comment}{$\!\rhd$ }
\newcommand{\Inparallel}{{\bf in parallel} }	%This should be flushed
\newcommand{\Goto}{{\bf goto} }
\newcommand{\Error}{{\bf error} } % optionally followed by string argument

\newcommand{\const}[1]{{\hbox{\sc#1}}}
\newcommand{\proc}[1]{{\hbox{\sc#1}}}

%\newcommand{\proc}[1]{%
%\ifmmode\mathord{\mathcode`-="702D\rm#1\mathcode`\-="2200}\else{\rm#1}\fi}
\newcommand{\procdecl}[1]{\proc{#1}\vrule width0pt height0pt depth 7pt \relax}
\newcommand{\id}[1]{\ifmmode\mathord{\mathcode`-="702D\mathit #1\mathcode`\-="2200}\else$\mathord{\mathcode`-="702D\mathit #1\mathcode`\-="2200}$\fi}
%\newcommand{\func}[1]{\ifmmode\mathop{\mathcode`-="702D\sc #1\mathcode`\-="2200}\nolimits\else$\mathop{\mathcode`-="702D\sc #1\mathcode`\-="2200}\nolimits$\fi}
\newcommand{\func}[1]{{\sc #1}}




==> mymacros.tex <==
\setlength\abovecaptionskip{1pt}
\setlength\belowcaptionskip{2pt plus 1pt minus 1pt}
\setlength{\floatsep}{6pt plus 5pt minus 2pt}
\setlength{\dblfloatsep}{6pt plus 5pt minus 2pt}
\setlength{\textfloatsep}{6pt plus 10pt minus 3pt}
\setlength{\dbltextfloatsep}{6pt plus 10pt minus 3pt}

\renewcommand{\topfraction}{0.9}
\renewcommand{\bottomfraction}{0.9}
\renewcommand{\textfraction}{0.1}
\renewcommand{\floatpagefraction}{0.9}

% \parskip 3pt plus 2pt minus 2pt    

% Added by rahuls to save space by eliminating space b/t paragraphs
%
\setlength{\parskip}{0in}
\setlength{\parindent}{1pc}
        
\makeatletter

\renewcommand{\ttdefault}{cmt}


\renewcommand{\section}{\@startsection
  {section}%
  {1}%
  {0mm}%
  {6pt plus 2pt}%
  {6pt plus 2pt}%
  {\normalfont\Large\bf}}

\renewcommand{\subsection}{\@startsection
  {subsection}%
  {2}%
  {0mm}%
  {4pt plus 2pt}%
  {4pt plus 2pt}%
  {\normalfont\large\bf}}

\renewcommand{\subsubsection}{\@startsection
  {subsubsection}%
  {3}%
  {0mm}%
  {2pt plus 2pt}%
  {2pt plus 2pt}%
  {\normalfont\normalsize\bf}}

\renewcommand{\paragraph}{\@startsection
  {paragraph}%
  {4}%
%  {0mm}%
  {4mm}%
  {2pt plus 2pt}%
  {-1em}%
  {\normalfont\normalsize\bf}}

\def\maketitle{\par
 \begingroup
   \def\thefootnote{\fnsymbol{footnote}}
   \def\@makefnmark{\hbox
       to 0pt{$^{\@thefnmark}$\hss}}
   \if@twocolumn
     \twocolumn[\@maketitle]
     \else \newpage
     \global\@topnum\z@         % Prevents figures from going at top of page.
%     \@maketitle \fi\thispagestyle{empty}\@thanks
     \@maketitle \fi\@thanks
 \endgroup
 \setcounter{footnote}{0}
 \let\maketitle\relax
 \let\@maketitle\relax
 }

\newenvironment{captiontext}{%
   \begin{center}%
     \begin{minipage}{0.9\linewidth}%
       \renewcommand{\baselinestretch}{0.9}%
         \sffamily\small}%
   {\renewcommand{\baselinestretch}{1.0}%
      \end{minipage}%
        \end{center}}

\newenvironment{smenumerate}%
  { \newcounter{foo_counter}
    \begin{list}{\arabic{foo_counter}}%
     {\usecounter{foo_counter}
      \setlength{\parsep}{0pt}%
      \setlength{\topsep}{0pt}%
      \setlength{\itemsep}{2pt}}}%
  {\end{list}}

\newenvironment{smitemize}%
  {\begin{list}{$\bullet$}%
     {\setlength{\parsep}{0pt}%
      \setlength{\topsep}{0pt}%
      \setlength{\itemsep}{2pt}}}%
  {\end{list}}

\newenvironment{sm1enumerate}%
  { \newcounter{foo_counter}
    \begin{small}\begin{list}{\arabic{foo_counter}}%
     {\usecounter{foo_counter}
      \setlength{\parsep}{0pt}%
      \setlength{\topsep}{0pt}%
      \setlength{\itemsep}{5pt}}}%
  {\end{list}\end{small}}

\newenvironment{sm1itemize}%
  {\begin{small}\begin{list}{$\bullet$}%
     {\setlength{\parsep}{0pt}%
      \setlength{\topsep}{0pt}%
      \setlength{\itemsep}{5pt}}}%
  {\end{list}\end{small}}


\newenvironment{ColVerb}%
	{\VerbatimEnvironment
	\begin{Sbox}\begin{minipage}{73mm}\begin{alltt}}%
	{\end{alltt}\end{minipage}\end{Sbox}
	\setlength{\fboxsep}{3mm}\fbox{\TheSbox}}

\newenvironment{PageVerb}%
	{\VerbatimEnvironment
	\begin{Sbox}\begin{minipage}{158mm}\begin{alltt}}%
	{\end{alltt}\end{minipage}\end{Sbox}
	\setlength{\fboxsep}{3mm}\fbox{\TheSbox}}

\newenvironment{abstracttext}{%
     \begin{minipage}{0.9\linewidth}%
       \renewcommand{\baselinestretch}{0.9}%
         \small}%
      {\renewcommand{\baselinestretch}{1.0}%
     \end{minipage}}


%\makeatletter
\long\def\unmarkedfootnote#1{{\long\def\@makefntext##1{##1}\footnotetext{#1}}}
\makeatother

% Use comment package instead.
%\newcommand{\comment}[1]{}


\newcommand{\addrcheck}{{\sc AddrCheck}}
\newcommand{\memcheck}{{\sc MemCheck}}
\newcommand{\taintcheck}{{\sc TaintCheck}}
\newcommand{\lockset}{{\sc LockSet}}



==> toggles/sections/0_abstract.tex <==
\begin{abstract}
Bandwidth compression can be an effective way to achieve higher
system performance and energy efficiency in modern data-intensive
applications by exploiting redundancy and data similarity. Prior works have
studied a variety of data compression techniques to improve both capacity
(e.g., of caches and main memory) and bandwidth utilization (e.g., of
the on-chip and off-chip interconnects). 
%I think we can trip it - 
%These works addressed two
%common shortcomings of generic compression: (i) latency, energy, and
%area overheads of compression/decompression, and (ii) hardware
%complexity to support variable data size. 
In this paper, we make a
new observation about energy-efficiency of communication when compression is applied.
While compression reduces the amount of transferred data, it leads to a substantial increase in the
number of \emph{bit toggles} (communication channel switchings from 0
to 1 or from 1 to 0). The increased toggle count increases the dynamic
energy consumed by on-chip and off-chip buses due to more frequent
charging and discharging of the wires. Our results show that the total bit
toggle count can increase on average from 20\% to 2.2$\times$ when compression is applied 
for some compression algorithms, depending on the application suite.  We
characterize and demonstrate this new problem across 242 GPU
applications and six different compression algorithms. To mitigate the
problem, we propose two new {\em toggle-aware compression} techniques:
{\em Energy Control} and {\em Metadata Consolidation}. These
techniques greatly reduce the bit toggle count impact of the data
compression algorithms we examine, while keeping most of their
bandwidth reduction benefits.
\end{abstract}



==> toggles/sections/2_1_gpu_background.tex <==

%\noindent{\bf GPU Architecture.}
A GPU consists of multiple simple cores, also called 
streaming-multiprocessors (SMs) in NVIDIA terminology. Our 
example architecture (shown in Figure~\ref{fig:architecture}) 
consists of 32 cores each with a SIMT width of 32, and 6 
memory controllers. Each core is associated with a private 
L1 data cache and read-only texture and constant caches 
along with a low latency shared memory. 
The cores and memory controllers are connected via crossbar 
and every memory controller is associated with a slice of the 
shared L2 cache. 

\begin{figure}[h!]
\centering
\vspace{-0.2cm}
\includegraphics[width=0.23\textwidth]{figures/background.pdf}
\caption{Baseline GPU architecture.}
\label{fig:architecture}
\vspace{-0.3cm}
\end{figure}


%\noindent{\bf Application Execution.}
A typical GPU application consists of many kernels. Each kernel is divided into groups
of threads, called thread-blocks (or cooperative thread arrays (CTAs)).
After a kernel is launched and its necessary data is copied to the GPU 
memory, the thread-block scheduler schedules available CTAs onto all the available cores~\cite{gpgpu-sim}.
Once the CTAs are launched on the cores, the warps associated 
with CTAs are scheduled onto its SIMT pipelines. Each of these cores is capable of concurrently 
executing many warps, where a warp is typically defined 
as a batch of 32 threads. The maximum number of warps that 
can be launched on a core depends on the available 
core resources (e.g., available shared 
memory, register file size etc.). \comm{To efficiently support such fine-grain 
multi-threading, each core is provided with large register file to hold all 
the contexts of simultaneously active threads.} 



\ignore{


{\bf 2) COMMENT: I will write more based on how much background we 
are giving while explaining our schemes}

{\bf 3) COMMENT: Feel free to change text as desired. Also, for background
picture; my papers has images. We can potentially try to reuse it or make another
one; let me know}


\todo{adwait}{Could you us out here?}
Explain GPU operation:

- SMs/SPs

- Warps

- FGMT

- Scheduler

Fig: Basic GPU architecture
}


==> toggles/sections/other_channels.tex <==
%\subsection{PCIe and SATA interfaces} 

For SATA and PCIe, data is transmitted in a serial fashion at much
higher frequencies than typical parallel bus interfaces. Bit toggles within
these high speed bus interfaces have different implications than that of on-chip
or off-chit buses. First, since data
is transmitted in a serial fashion, data alignment at larger byte sizes no
longer plays a significant role in determining toggle rate. Second, bit toggles in
themselves, impose different design considerations and implications. Data is
transmitted across these buses without an accompanying clock signal which means
that the transmitted bits need to be synchronized with a clock signal by the
receiver. This \emph{clock recovery} requires \emph{frequent} bit toggles to
prevent loss in information. In addition, it is desirable that the \emph{running
disparity}{\textemdash}which is the difference in the number of one and zero
bits transmitted{\textemdash}be minimized. This condition is referred to as
\emph{DC balance} and prevents distortions in the signal. Data is typically
scrambled using encodings like the 8b/10b encoding~\ref{8b10b} to balance the
number of ones and zeros while ensuring frequent transitions. These
encodings have high overhead in terms of the amount of additional data
transmitted but obscure any difference in bit transitions with compressed or
uncompressed data. We do not expect that the changed data after compression would pose any additional
challenges to these interfaces, and hence we do not apply our proposed techniques
to SATA and PCIe, and just provide their description for the overview completeness.  

